Re-Examining Calibration: The Case of Question Answering

For users to trust model predictions, they need to understand model outputs, particularly their confidence - calibration aims to adjust (calibrate) models' confidence to match expected accuracy. We argue that the traditional calibration evaluation does not promote effective calibrations: for example, it can encourage always assigning a mediocre confidence score to all predictions, which does not help users distinguish correct predictions from wrong ones. Building on those observations, we propose a new calibration metric, MacroCE, that better captures whether the model assigns low confidence to wrong predictions and high confidence to correct predictions. Focusing on the practical application of open-domain question answering, we examine conventional calibration methods applied on the widely-used retriever-reader pipeline, all of which do not bring significant gains under our new MacroCE metric. Toward better calibration, we propose a new calibration method (ConsCal) that uses not just final model predictions but whether multiple model checkpoints make consistent predictions. Altogether, we provide an alternative view of calibration along with a new metric, re-evaluation of existing calibration methods on our metric, and proposal of a more effective calibration method.

==> scripts/git-latexdiff <==
#! /bin/bash

# Main author: Matthieu Moy <Matthieu.Moy@imag.fr> (2012 - 2016)
# (See the Git history for other contributors)
#
# Copying and distribution of this file, with or without modification,
# are permitted in any medium without royalty provided the copyright
# notice and this notice are preserved.  This file is offered as-is,
# without any warranty.
#
# git-latexdiff is a wrapper around latexdiff
# (http://www.ctan.org/pkg/latexdiff) that allows using it to diff two
# revisions of a LaTeX file.
#
# The script internally checks out the full tree for the specified
# revisions, calls latexpand to flatten the document and then calls
# latexdiff, hence this works if the document is split into multiple
# .tex files.
#
# Try "git latexdiff -h" for more information.
#
# To install, just copy git-latexdiff in your $PATH.

# Missing features (patches welcome ;-):
# - diff the index
# - hardlink temporary checkouts as much as possible

# Alternatives:
#
# There is another script doing essentially the same here:
# https://github.com/cawka/latexdiff/blob/master/latexdiff-git
# My experience is that latexdiff-git is more buggy than
# git-latexdiff, but they probably just don't have the same bugs ;-)
#
# There are a bunch of other alternatives cited here:
#
#   http://tex.stackexchange.com/questions/1325/using-latexdiff-with-git
#
# Ideally, these scripts should be merged.

set -o errexit
set -o noclobber

# Some versions of git set $GIT_WORK_TREE when ran through an alias.
# This wouldn't work with git-latexdiff which plays with different
# work trees.
unset GIT_DIR
unset GIT_WORK_TREE

# (Comment and 'unset' line borrowed from Git's source code)
# Having this variable in your environment would break scripts because
# you would cause "cd" to be taken to unexpected places.  If you
# like CDPATH, define it for your interactive shell sessions without
# exporting it.
# But we protect ourselves from such a user mistake nevertheless.
unset CDPATH

# @GIT_LATEXDIFF_VERSION@ is substituted by the install script here,
# but not within git_latexdiff_compute_version().
git_latexdiff_version='@GIT_LATEXDIFF_VERSION@'

git_latexdiff_compute_version () {
    if [ "$git_latexdiff_version" = '@GIT_LATEXDIFF''_VERSION@' ]; then
	(cd "$(dirname "$0")" && git describe --tags HEAD 2>/dev/null || echo 'Unknown version')
    else
	echo "$git_latexdiff_version"
    fi
}

usage () {
    cat << EOF
Usage: $(basename "$0") [options] OLD [NEW]
       $(basename "$0") [options] OLD --
       $(basename "$0") [options] -- OLD
Call latexdiff on two Git revisions of a file.

OLD and NEW are Git revision identifiers. NEW defaults to HEAD.
If "--" is used for NEW, then diff against the working directory.

Options:
    --help                this help message
    --main <file.tex>     name of the main LaTeX file
    --no-view             don't display the resulting PDF file
    --latex               run latex instead of pdflatex
    --bibtex, -b          run bibtex as well as latex
                             (pdflatex,bibtex,pdflatex,pdflatex)
    --biber               run BibLaTex-Biber as well as latex
                             (pdflatex,bibtex,pdflatex,pdflatex)
    --view                view the resulting PDF file
                            (default if -o is not used)
    --pdf-viewer <cmd>    use <cmd> to view the PDF file (default: \$PDFVIEWER)
    --no-cleanup          don't cleanup temp dir after running
    --no-flatten          don't call latexpand to flatten the document
    --cleanup MODE        Cleanup temporary files according to MODE:

                           - keeppdf (default): keep only the
                                  generated PDF file

                           - none: keep all temporary files
                                  (may eat your diskspace)

                           - all: erase all generated files.
                                  Problematic with --view when the
                                  viewer is e.g. evince, and doesn't
                                  like when the file being viewed is
                                  deleted.

    --latexmk             use latexmk
    --latexopt            pass additional options to latex (e.g. -shell-escape)
    -o <file>, --output <file>
                          copy resulting PDF into <file> (usually ending with .pdf)
                          Implies "--cleanup all"
    --tmpdirprefix        where temporary directory will be created (default: /tmp)
    --verbose, -v         give more verbose output
    --quiet               redirect output from subprocesses to log files
    --prepare <cmd>       run <cmd> before latexdiff (e.g. run make to generate
                             included files)
    --ln-untracked        symlink uncommited files from the working directory
    --version             show git-latexdiff version.
    --subtree             checkout the tree at and below the main file
                             (enabled by default, disable with --whole-tree)
    --whole-tree          checkout the whole tree (contrast with --subtree)
    --ignore-latex-errors keep on going even if latex gives errors, so long as
                          a PDF file is produced
    --ignore-makefile     ignore the Makefile, build as though it doesn't exist
    -*                    other options are passed directly to latexdiff
    --bbl                 shortcut to flatten a bbl file of the same name as the project
    --latexpand           pass options to latexpand (should be last option specified)
    --latexdiff-flatten   use --flatten from latexdiff instead of latexpand
EOF
}

die () {
    echo "fatal: $*"
    exit 1
}

verbose () {
    if test "$verbose" = 1 ; then
	printf "%s ..." "$@"
    fi
}

verbose_progress () {
    if test "$verbose" = 1 ; then
	printf "."
    fi
}

verbose_done () {
    if test "$verbose" = 1 ; then
	echo " ${1:-done}."
    fi
}

verbose_say () {
    if test "$verbose" = 1 ; then
	printf "%s\n" "$@"
    fi
}

old=
new=
main=
view=maybe
cleanup=keeppdf
verbose=0
bibtex=0
biber=0
output=
initial_dir=$PWD
initial_repo=$(git rev-parse --show-toplevel)
tmpdir_prefix="/tmp"
prepare_cmd=
flatten=1
subtree=1
uselatexmk=
latexopt=
ln_untracked=0
quiet=0
ignorelatexerrors=0
latexdiffopt=()
latexpand=()
bbl=0
latexdiff_flatten=0
latex=0


while test $# -ne 0; do
    case "$1" in
        "--help"|"-h")
            usage
            exit 0
            ;;
	"--main")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    main=$1
	    ;;
	"--no-view")
	    view=0
	    ;;
	"--view")
	    view=1
	    ;;
	"--pdf-viewer")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    PDFVIEWER="$1"
	    ;;
	"--no-cleanup")
	    cleanup=none
	    ;;
	"--ignore-latex-errors")
	    ignorelatexerrors=1
	    ;;
        "--cleanup")
            shift
            case "$1" in
                "none"|"all"|"keeppdf")
                    cleanup="$1"
                    ;;
                *)
                    echo "Bad argument --cleanup $1"
                    usage
                    exit 1
                    ;;
            esac
            ;;
	"--no-flatten")
            flatten=0
            ;;
	"--ignore-makefile")
	    ignoremake=1
	    ;;
	"-o"|"--output")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    output=$1
	    cleanup=all
	    ;;
	"-b"|"--bibtex")
	    bibtex=1
	    ;;
	"--latex")
	    latex=1
	    ;;
	"--biber")
	    biber=1
	    ;;
	"--verbose"|"-v")
	    verbose=1
	    ;;
        "--quiet")
	    quiet=1
	    ;;
	"--version")
	    git_latexdiff_compute_version
            exit 0
	    ;;
	"--subtree")
	    subtree=1
	    ;;
	"--whole-tree")
	    subtree=0
	    ;;
	"--prepare")
	    shift
	    prepare_cmd="$1"
	    ;;
        "--latexmk")
            uselatexmk=1
            ;;
	"--latexpand")
	    shift
	    latexpand=$1
	    ;;
	"--bbl")
	    bbl=1
	    ;;
	"--latexdiff-flatten")
	    latexdiff_flatten=1
            flatten=0
	    ;;
	"--latexopt")
	    shift
	    latexopt=$1
	    ;;
        "--ln-untracked")
            ln_untracked=1
            ;;
        "--no-ln-untracked")
            ln_untracked=0
            ;;
        "--tmpdirprefix")
	    shift
	    tmpdir_prefix="$1"
	    ;;
        -*)
            if test "$1" = "--" ; then
                if test -z "$new" ; then
                    new=$1
                else
                    echo "Bad argument $1"
                    usage
                    exit 1
                fi
            else
                latexdiffopt+=("$1")
            fi
            ;;
        *)
	    if test -z "$1" ; then
		echo "Empty string not allowed as argument"
		usage
		exit 1
	    elif test -z "$old" ; then
		old=$1
	    elif test -z "$new" ; then
		new=$1
	    else
		echo "Bad argument $1"
		usage
		exit 1
	    fi
            ;;
    esac
    shift
done

if test -z "$new" ; then
    new=HEAD
fi
if test "$new" = "--"; then
    ln_untracked=1
fi

if test -z "$old" ; then
    echo "fatal: Please, provide at least one revision to diff with."
    usage
    exit 1
fi

if test -z "$PDFVIEWER" ; then
    verbose "Auto-detecting PDF viewer"
    candidates="xdg-open evince okular xpdf acroread"
    if test "$(uname)" = Darwin ; then
        # open exists on GNU/Linux, but does not open PDFs
	candidates="open $candidates"
    fi

    for command in $candidates; do
	if command -v "$command" >/dev/null 2>&1; then
	    PDFVIEWER="$command"
	    break
	else
	    verbose_progress
	fi
    done
    verbose_done "$PDFVIEWER"
fi

case "$view" in
    maybe|1)
	if test -z "$PDFVIEWER" ; then
	    echo "warning: could not find a PDF viewer on your system."
	    echo "warning: Please set \$PDFVIEWER or use --pdf-viewer CMD."
	    PDFVIEWER=false
	fi
	;;
esac

if test $flatten = 1 &&
    ! command -v latexpand 2>/dev/null; then
    echo "Warning: latexpand not found. Falling back to latexdiff --flatten."
    latexdiff_flatten=1
    flatten=0
fi

if test $latex = 1; then
    LATEX_EXEC=latex
else
    LATEX_EXEC=pdflatex
fi    

## end option parsing ##

check_knitr () {
    if test -z "$prepare_cmd"; then
	prepare_cmd="Rscript -e \"library(knitr); knit('$main')\""
    fi
    main="${main%\.*}.tex"
}

log_cmd () {
    log=$1
    shift
    if [ "$quiet" = 1 ]; then
	"$@" >$log 2>&1
    else
	"$@"
    fi
}

# main is relative to initial_dir (if returned)
if test -z "$main" ; then
    printf "%s" "No --main provided, trying to guess ... "
    main=$(git grep -l '^[ \t]*\\documentclass')
    # May return multiple results, but if so the result won't be a file.
    if test -r "$main" ; then
	echo "Using $main as the main file."
    else
	if test -z "$main" ; then
	    echo "No candidate for main file."
	else
	    echo "Multiple candidates for main file:"
	    printf "%s\n" "$main" | sed 's/^/\t/'
	fi
	die "Please, provide a main file with --main FILE.tex."
    fi
fi

ext=${main##*\.}
case "$ext" in
    Rnw) check_knitr ;;
    Rtex) check_knitr ;;
    *) ;;
esac

if test ! -r "$main" ; then
    die "Cannot read $main."
fi

verbose "Creating temporary directories"

git_prefix=$(git rev-parse --show-prefix)
git_dir="$(git rev-parse --git-dir)" || die "Not a git repository?"
cd "$(git rev-parse --show-cdup)" || die "Can't cd back to repository root"
git_dir=$(cd "$git_dir"; pwd)

# make main relative to git root directory
if test -n "$git_prefix" ; then
    main=$git_prefix$main
fi
mainbase=$(basename "$main" .tex)
maindir=$(dirname "$main")

tmpdir=$tmpdir_prefix/git-latexdiff.$$
mkdir "$tmpdir" || die "Cannot create temporary directory."

cd "$tmpdir" || die "Cannot cd to $tmpdir"

mkdir old new || die "Cannot create old and new directories."

verbose_done
verbose_say "Temporary directories: $tmpdir/old and $tmpdir/new"
verbose "Checking out old and new version"

cd old || die "Cannot cd to old/"
if test "$ln_untracked" = 1; then
    (
       mkdir -p "$maindir" && cd "$maindir" && ln -s "$initial_repo"/"$maindir"/* .
    )
fi

if test "$subtree" = 1; then
    checkoutroot=$git_prefix
else
    checkoutroot="."
fi

# Checkout a subtree, without touching the index ("git checkout" would)
(cd "$git_dir" && git archive --format=tar "$old" "$checkoutroot") | tar -xf -
verbose_progress
cd ../new || die "Cannot cd to new/"
if test "$ln_untracked" = 1; then
    (
       mkdir -p "$maindir" && cd "$maindir" && ln -s "$initial_repo"/"$maindir"/* .
    )
fi
if test "$new" != "--"; then
    # if new == "--" then diff working dir (already there thanks to ln
    # -s above).
    (cd "$git_dir" && git archive --format=tar "$new" "$checkoutroot") | tar -xf -
fi
verbose_progress
cd ..

verbose_done

for dir in old new
do
    verbose "Running preparation command $prepare_cmd in $dir/$git_prefix"
    ( cd "$dir/$git_prefix/" && log_cmd prepare.log eval "$prepare_cmd" )
    if test ! -f "$dir/$main"; then
	die "$prepare_cmd did not produce $dir/$main."
    fi
    verbose_done
done

# Option to use latexdiff --flatten instead of latexpand
if test "$latexdiff_flatten" = 1; then
    latexdiffopt+=("--flatten")
fi

# Shortcut to include bbl
if test "$bbl" = 1; then
    bblexpand=("--expand-bbl" "$mainbase.bbl")
else
    bblexpand=()
fi

# Create flattened documents and keep for debugging
if test "$flatten" = 1; then
    if [ "$bbl" = 1 ]; then
	if [ ! -f "old/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing old/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd old/"$maindir"
	    log_cmd pdflatex0.log pdflatex $latexopt "$mainbase" || compile_error=1
	    log_cmd bibtex0.log bibtex "$mainbase" || compile_error=1
	    cd "$oldPWD"
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for old version"
	    fi
	fi
	if [ ! -f "new/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing new/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd new/"$maindir"
	    log_cmd pdflatex0.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
	    log_cmd bibtex0.log bibtex "$mainbase" || compile_error=1
	    cd "$oldPWD"
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for new version"
	    fi
	fi
    fi
    verbose "Running latexpand"
    (
	cd old/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > old-"$mainbase"-fl.tex \
	|| die "latexpand failed for old version"
    (
	cd new/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > new-"$mainbase"-fl.tex \
	|| die "latexpand failed for new version"
    verbose_done

    verbose "Running latexdiff ${latexdiffopt[*]} old-${mainbase}-fl.tex new-${mainbase}-fl.tex > ./diff.tex"
    latexdiff "${latexdiffopt[@]}" old-"$mainbase"-fl.tex new-"$mainbase"-fl.tex > diff.tex \
	|| die "latexdiff failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new-"$mainbase"-fl.tex new-"$mainbase"-fl.tex.orig
    mv -f diff.tex new/"$main"
    verbose_done
else
    verbose "Running latexdiff ${latexdiffopt[*]} old/$main new/$main > ./diff.tex"
    latexdiff "${latexdiffopt[@]}" old/"$main" new/"$main" > diff.tex \
	|| die "latexdiff failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new/"$main" new/"$main.orig"
    mv -f diff.tex new/"$main"
    verbose_done
fi

verbose "Compiling result"

compile_error=0
cd new/"$maindir" || die "Can't cd to new/$maindir"
if test -f Makefile && test "$ignoremake" != 1 ; then
    log_cmd make.log make || compile_error=1
elif test "$uselatexmk" = 1; then
    log_cmd latexmk.log latexmk -f -pdf -silent "$mainbase" || compile_error=1
else
    if [ "$ignorelatexerrors" = 1 ]; then
	latexopt="$latexopt -interaction=batchmode"
    elif [ "$quiet" = 1 ]; then
	latexopt="$latexopt -interaction=nonstopmode"
    else
	latexopt="$latexopt -interaction=errorstopmode"
    fi
    log_cmd pdflatex1.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
    if test "$bibtex" = 1 ; then
	log_cmd bibtex.log bibtex "$mainbase" || compile_error=1
    fi
    if test "$biber" = 1 ; then
	log_cmd biber.log biber "$mainbase" || compile_error=1
    fi
    log_cmd pdflatex2.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
    log_cmd pdflatex3.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
fi

verbose_done

if [ "$compile_error" = 1 ] && [ "$ignorelatexerrors" = 1 ]; then
    echo "LaTeX errors were found - but attempting to carry on."
    compile_error=0
fi

if test $latex = 1; then
    dvips "$mainbase".dvi
    ps2pdf "$mainbase".ps
fi

pdffile="$mainbase".pdf
if test ! -r "$pdffile" ; then
    echo "No PDF file generated."
    compile_error=1
fi

if test ! -s "$pdffile" ; then
    echo "PDF file generated is empty."
    compile_error=1
fi

if test "$compile_error" = "1" ; then
    echo "Error during compilation. Please examine and cleanup if needed:"
    echo "Directory: $tmpdir/new/$maindir"
    echo "     File: $mainbase.tex"
    # Don't clean up to let the user diagnose.
    exit 1
fi

if test -n "$output" ; then
    abs_pdffile="$PWD/$pdffile"
    (cd "$initial_dir" && mv "$abs_pdffile" "$output")
    echo "Output written on $output"
elif [ -f "$pdffile" ]; then
    new_pdffile="$tmpdir"/"$pdffile"
    mv "$pdffile" "$new_pdffile"
    pdffile="$new_pdffile"
fi


if test "$view" = 1  || test "$view" = maybe  && test -z "$output" ; then
    "$PDFVIEWER" "$pdffile"
fi

case "$cleanup" in
    "all")
	verbose "Cleaning-up result"
	cd ..
	cd ..
	rm -fr "$tmpdir"
	verbose_done
	;;
    "keeppdf")
	verbose "Cleaning-up all but pdf (kept in $pdffile)"
	rm -fr "$tmpdir"/old "$tmpdir"/new
	verbose_done
	;;
    "none")
	verbose_say "Generated files kept in $tmpdir/"
	;;
esac


==> scripts/style-check/bad-words <==
utilize              % phrase "use" http://www.bartleby.com/64/C003/0294.html
utilizes             % phrase "uses" http://www.bartleby.com/64/C003/0294.html
utilized             % phrase "used" http://www.bartleby.com/64/C003/0294.html
utilizing            % phrase "using" http://www.bartleby.com/64/C003/0294.html
leverage             % phrase "use"
abstraction          % phrase this is often used poorly?
fashion              % phrase hrm.
[dw]on't             % spelling do not or will not.
behavioral           % spelling I'm convinced we don't use this word properly.
we'll                % spelling we will
we've                % spelling we have
[^r][^c][^h] impact  % phrase "consequences", "effect", "result", though nsf likes "research impact"
tackle               % phrase "tackle" (a problem) is wimpy for "solve" or a tired metaphor for "address a challenge".
thusly               % phrase "thus" or "this way" or "like this" http://www.bartleby.com/64/C003/0282.html
transpire            % phrase "happen" 
so-called            % phrase can be abused; it's negative.
necessitate          % phrase require.
necessitated         % phrase required.
necessitates         % phrase requires.
loosing              % spelling you almost certainly mean "losing".  use "loosening" otherwise.
aforementioned       % phrase too pretentious.
important to         % phrase "valued by"?
notion               % phrase avoid this weak phrase. (thanks brian bershad!)
achieve(s)?\s        % phrase models don't achieve anything, only use for humans
reasonably           % phrase hedging


==> scripts/style-check/common-typos <==
a the                % phrase double article
 pt                  % syntax ? I guess avoid straggling pt's that escape tex?
[ ],                 % syntax whitespace before comma seems wrong.
Figure Figure        % phrase pizza pizza.
[ ]-[ ]              % syntax a hyphen surrounded by space should probably be an emdash '---'
[0-9]-[0-9]          % syntax use an endash '--' for ranges
[0-9]ms              % syntax put a space between the number and the unit.
[^egs]\. [a-z]       % syntax a period usually ends a sentence, and sentences should start with a capital; doesn't apply for i.e.,
\.  [a-z]            % syntax a period usually ends a sentence, and sentences should start with a capital; "i.e." should have a comma following.
[a-z]\.\.            % syntax double period is rarely right, use \ldots for ellipsis
[^\\]"               % syntax use fancy quotes
\beg\.               % syntax should be e.g. as in "examples given"
from to\b            % phrase haven't used this properly.
help help            % phrase double word, that probably means the author paniced
of of                % phrase apparent double word.
the affect           % phrase should probably be 'the effect'
the the              % phrase apparent double word.
there too few        % phrase there are too few?
was not was          % phrase pretty much a joke if this gets matched.
we we                % phrase it would be oi oi in french, I guess.
with on              % phrase probably wrong.
with with            % phrase apparent double word.
[\n ]--[\n ]         % syntax that's an en-dash, you want an em-dash: "---"
my my                % phrase unlikely that's what you want, at least without a comma. (doesn't work across newlines)
>From                % syntax be careful when you email .tex files.  I've seen this slip through into submissions.
e\.t\.c\.            % syntax it's et cetera; use etc.
such as like         % phrase pick one
<<<<<<< .            % syntax CVS conflict!
=======              % syntax CVS conflict!
>>>>>>> [0-9]        % syntax CVS conflict!
e\.g\.[\n ]          % syntax should be followed with a comma, as e.g. can be read as "for example" (thanks JZ!)
i\.e\.[\n ]          % syntax should be followed with a comma, as i.e. can be read as "that is" (thanks JZ!)
[ ]\.[\n ]           % syntax stray period?
further more         % phrase one word: furthermore
safe guard           % phrase one word: safeguard
that be              % phrase mistake.
can not              % phrase cannot
only only            % phrase double word
is is                % phrase double word.
they shows           % phrase argh, mistake.
less that than       % phrase typo damage
from from            % phrase double word score
in in                % phrase "in" (common mistake)
not not              % phrase argh.
it it                % phrase argh.
to illicit           % phrase "to elicit" -- illicit is always an adjective.
c\.f\.               % phrase actually, it's cf., and you'd like cf.\ (backslash space)
this lead to         % phrase "led to" if past tense, "leads to" if present.
on on                % phrase double word.
has is               % phrase choose
description their    % phrase saw this, clearly wrong.
including:  % syntax I prefer no colon after including, which already says a list is coming.
[a-z]\([A-Z]  % syntax put a space before parens, even when introducing acronyms.
without and without % phrase saw this.
can be result       % phrase saw this typo.



==> scripts/style-check/foolish-phrases <==
(quite|more|very|most) unique    % phrase unique is.
(quite|more|very|most) abstract  % phrase abstract is.
tangible view                    % phrase mix that metaphor some more.
for e\.g\.                       % phrase e.g. includes "for".
begs the question                % phrase unless you're very clever: "raises the question": http://alt-usage-english.org/excerpts/fxbegthe.html
high rate of speed               % phrase local news-speak.
especially necessary             % phrase 'especially important', necessary may be an absolute like unique.
how will it effect % phrase you likely meant "affect"
how it will effect % phrase you likely meant "affect"
insure proper performance % phrase "ensure"
especially true                  % phrase 'especially important', true may be an absolute like unique.
to affect change                 % phrase "effect" change;  I read this on a poster.
higher results                   % phrase maybe higher performance or higher values.
is more general then the         % phrase probably "than"
upper bounding                   % phrase "limiting" or "setting an upper bound on"
in principal                     % phrase likely, "in principle"
literally like                   % phrase literally means no simile.  
design principal  % phrase likely, "design principle" 
different from 	    	   	 % phrase unlike

==> scripts/style-check/latex-checking <==
\{\\em [^\}]*[^\}\/]\}[:]    % syntax use \emph{} or explicit italic correction {\em foo\/}
\{\\em [^\}]*[:\.,]\}        % syntax punctuation at the edges of italic text is not italicized
[A-Z]{2,10}\.[ ]*[\n ][ ]*[A-Z]  % syntax intersentence spacing should be used if a sentence ends with an acronym: "FOO\\@."
\\etal[^{]                   % syntax it's good practice to use \etal{} to avoid bad spacing
\\caption\[[^\]]*[^\.]\]     % syntax short caption should end with a period.
\\caption\[.*CCDF.*\]        % syntax short caption should not include graph type.
\\caption\[.*CDF.*\]         % syntax short caption should not include graph type.
\\caption\[.{0,25}\]         % syntax short caption should not be too short.
th century                   % syntax use textsuperscript
[ ]---[ ]                    % syntax the em-dash should be right up against the words.
[ \n]---[ \n]                % syntax the em-dash should be right up against the words.
^---[ \n]                    % syntax the em-dash should be right up against the words.
[ \n]---$                    % syntax the em-dash should be right up against the words.
[ \n]--[ \n]                 % syntax the en-dash should be between numbers.
^--[ \n]                     % syntax the en-dash should be between numbers.
[ \n]--$                     % syntax the en-dash should be rbetween numbers.
,[~ ]\\etal                  % syntax no comma before etal (unless Smith, Martinez, \etal)
\\etal\{\}'s                 % syntax eew.
\\(sub)?section\{[A-Z][^}]*[ ][a-z]{5,40}[^}]*\} % syntax subsection headers should be initial capped.
\\(sub)?section\{[A-Z][^}]*[^:][ ]{1,}(With|A|An|Is|And|For|To|The)[ ][^}]*\} % syntax some words needn't be capitalized
[ ]\\footnote                % syntax no space before footnote.
\\footnote\{.*\}.            % syntax footnotes after punctuation
,,                           % syntax double comma is unlikely to be intentional.
cf\.[^\\]                    % phrase cf. should get an escaped space "\ "
et al\.[^\\]                    % phrase et al. should get an escaped space "\ "
[<>]  % syntax a less than or greater than outside math mode shows other characters.
in (section|table|figure) \\ref % phrase should have ~ before ref
section~\\ref % capitalize capitalize section when saying Section 6.
table~\\ref % capitalize capitalize section when saying Table 6.
figure~\\ref % capitalize capitalize section when saying Figure 6.
\\(sub)?section\{Intro\} % syntax spell it out.
,''                          % syntax punctuation outside quotes
\.\.\.                       % syntax use \dots

==> scripts/style-check/my-rules <==
#  such may be abused to blacklist certain words even spelled correctly.
# capitalize is case sensitive, and also bracketed by non-word.
# phrase and spelling are case insensitive, but bracketed by non-word characters.
# syntax is case sensitive but not bracketed by non-word; probably best if used with regexes.
\bet al\.[^}]        % syntax use the \etal{} command instead. (or write one to italicize)
\bet\. al\.          % syntax use the \etal{} command, "et" needs no dot (et alii). (or write one to italicize)
\bc\.f\.\b             % syntax should be cf. for "confer" (latin for compare)
\b$i\)[^$]              % syntax leave the paren in math mode -- should be $i)$
\b$ii\)[^$]             % syntax leave the paren in math mode -- should be $ii)$
\b$iii\)[^$]            % syntax leave the paren in math mode -- should be $iii)$
\b$iv\)[^$]             % syntax leave the paren in math mode -- should be $iv)$
\b$v\)[^$]              % syntax leave the paren in math mode -- should be $v)$
\ban [b-df-gj-np-tv-z] % syntax probably meant to use "a" instead of "an", though there are exceptions.
\ban [B-DF-GJ-NP-TV-Z][^A-Z/] % syntax probably meant to use "a" instead of "an", though there are exceptions (like acronyms).
\b[Aa] [aeiouAEIOU](?!se|ni|A|ur|RL|ti|ne|DP) % syntax probably meant to use "an" instead of "a", though there are exceptions. (user, useful, AA, unified, uniform, unique, Europe, one, UDP; n/a doesn't work, so use {n/a})
This allows           % phrase tie more explicitly: This (x) allows...
we find               % phrase omit "we find"
we found              % phrase omit "we found"
try and               % phrase "try to", though if you're using try as a noun in a compound sentence, this rule is wrong.
impact of             % phrase not a useful metaphor; try evaluation, success, effect, value.
including [^\.]*etc\. % syntax "including" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
includes [^\.]*etc\.  % syntax "includes" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
and etc\.             % phrase come on. learn some latin.
AT&T                  % syntax you poor thing, this won't compile.
doesn't               % phrase be formal.
be occur              % phrase what happens when I'm indecisive about what follows "can"
up until              % phrase "until"
one or more           % phrase probably redundant -- nonzero is probably implied.
is comprise(d|s) of   % phrase you probably mean "is composed of" because "comprises" is more a synonym for "contains" 
will be significantly different % phrase "will differ significantly" for active voice
More importantly,     % phrase probably means the order is wrong: put important stuff first.
todo                  % ignoredcommand
texttt                  % ignoredcommand
jbgcomment              % ignoredcommand
lkfcomment              % ignoredcommand
due to space constraints % phrase don't whine.
this paper % phrase can be ambiguous if talking about someone else's paper whether you mean the one youre writing or the one you're talking about..
the above             % phrase horrible phrase that must be expunged.  you might use "these" instead, but best to make the sentence stand alone.
referred to above     % phrase "these".
(all|the|of) [0-9][ ] %  phrase use words for numbers in phrases.
clearly shows         % phrase "clearly" is usually much.
grows larger          % phrase is "grows smaller" possible?  grows.
guarantee as much as possible % phrase then not really a guarantee "provide"
affects negatively   % phrase "hurts" or "harms"
rely upon % phrase rely on is good enough
relies upon % phrase relies on is good enough
record route packets? % phrase hyphenate record-route packets
record-route; % phrase leave record route alone if not modifying something else
we accomplish this  % phrase verbose way to get active voice.
refers to the % phrase you're being wimpy in the definition.  use "is"
\\emph\{[a-zA-Z ]*\} refers to % syntax you're being wimpy in the definition.
loss off % phrase loss of?
this could % phrase this "what" could
with that has % phrase probably just one
simply % phrase probably isn't.
to get to % phrase "to reach"?
latency benefit % phrase reduction
latency improvement % phrase reduction
shed insight % phrase 'shed light' would seem the metaphor.
increasingly more % phrase redundant
I\.e\. % syntax starting a sentence with i.e. is just ugly.
E\.g\. % syntax starting a sentence with e.g. is just ugly.
in the large % phrase if large is a noun, bad.  if it's an adjective, fine.
encapsulates with % phrase seen it, don't know what it means.
when working with % phrase just say "with"
it is true that	  % phrase usually can delete
LDA % phrase convention put in small caps
(F|f)indings (show|indicate|suggest)	% phrase delete or make more specific

==> scripts/style-check/networking-research <==
IPs                  % phrase should be IP addresses
[Rr]ate-limits       % spelling "rate limits" has no hyphen, only "rate-limited"
best effort          % phrase hyphenate best-effort service.
deliver route        % phrase jargon redundancy
euclidean % capitalize Euclidean.
interdomain          % spelling inter-domain
internet             % capitalize unless talking about an internet other than the Internet
intradomain          % spelling intra-domain
log-normal           % spelling lognormal is one word.
pareto               % capitalize
ttl                  % capitalize
weibull              % capitalize proper name.
PoP                  % syntax I think POP looks less annoying.
PoPs                 % syntax I think POP looks less annoying.
http[ ]              % capitalize capitalize HTTP.
linux                % capitalize capitalize Linux
Internet[^\.]*Internet % syntax avoid Internet twice in the same sentence?
zipf                 % capitalize capitalize the guy's name.


==> scripts/style-check/passive-voice <==
it is possible to                   % phrase passive voice, try: "can"
are identified by                   % phrase passive
is shown                            % phrase passive.
is not included in                  % phrase maybe this is passive
there (are|is) [^\.:;]* (that|in)   % phrase maybe this is passive
can be evaluated                    % phrase avoid passive: I evaluated
can be observed                     % phrase avoid passive: are visible
# is needed                         % phrase passive voice
is used to                          % phrase go active voice, or subsititute "helps"
(are|were) needed[^\?]              % phrase passive voice
(is|are) presented in               % phrase "appears in", or reword to avoid passive voice
it is possible that                 % phrase "may"
(is|are) (depicted|illustrated|sketched) in  % phrase thats passive voice
(is|are) shown in                   % phrase "shows"
as can be seen in                   % phrase X shows that Y.
there needs to be                   % phrase passive voice in a bad way.
was designed                        % phrase passive voce.
it may be                           % phrase passive "it"
it is important that                % phrase passive; replace with X is important because Y.


==> scripts/style-check/verbose-phrases <==
a large number of                   % phrase you mean "many"
a substantial number of             % phrase how substantial?  most?  or just enough that can't be ignored?
an insufficient number of           % phrase "too few"
a significant number of             % phrase one is significant.   consider "prohibitive" if the number is sufficient to be problematic.
a number of                         % phrase getting the verb agreement for this useless phrase is tricky.
a number of different               % phrase use "different" (should have a high score)
a small number of                   % phrase you mean "few"
a low number of                   % phrase you mean "few"
a relatively low number of                   % phrase you mean "few"
actually                            % spelling probably doesn't add
to an extent                        % phrase you can probably remove
and instead                         % phrase replace with but?
be done                             % phrase if "X of Y can be done", try "Y can be Xed"; it's already passive voice.
combining multiple                  % phrase as opposed to "combining one?"
aggregating multiple                % phrase "aggregating"
do this                             % phrase probably verbose if you use a pronoun for what you're doing
exists[ ]                           % phrase probably no better than "is", but end of sentence may be unavoidable?
if it is to                         % phrase should be "to" (usually followed by "be X")
if they are to                      % phrase should be "to" (usually followed by "be X")
in general                          % phrase unless matched with "in specific," this is usually useless; perhaps "overall"
in order to                         % phrase remove "in order" and get "to"
in the past                         % phrase past tense is likely enough.
in the way of                       % phrase should be "as"
counting the number of              % phrase counting.  dude.
is permitted to                     % phrase "may"
largely opaque                      % phrase largely does not modify opaque
makes a new                         % phrase should be "creates"
may not chose                       % phrase "may not" is future tense; "chose" is past.
one should note                     % phrase just write it.
note that                           % phrase is the rest of the paper less notable?
Note, that                          % syntax not only should you not "note that", no comma after note.
we note                             % phrase is the rest of the paper less notable?
note however that                   % phrase is the rest of the paper less notable?
it is important to note             % phrase is the rest of the paper less notable?
really                              % phrase probably doesn't add; if you think it does, use "r{}eally" -- don't change to 'in fact'
in fact				    % phrase cut
rigorously                          % spelling probably doesn't add, and I rarely do anything with rigor
the way in which                    % phrase should be "how" or ""
the manner in which                 % phrase should be "how" or ""
value stems                         % phrase value is derived or offered, I think.
time at which                       % phrase very likely "when"
place at which                      % phrase very likely "where"
at the time                         % phrase very likely "when"
reduced number of                   % phrase very likely "fewer" or maybe maybe "less"
is present in                       % phrase present is probably redudant, try "is in"
they all                            % phrase maybe "all xs" would be better.
easy to do                          % phrase "feasible" or "practical" might be better.
is going to                         % phrase "will".
are going to                        % phrase "will".
getting                             % phrase probably "receiving" or "querying"
those are                           % phrase see if "those X are" is clearer?
design is motivated                 % phrase "inspired by" is probably better than "motivated" for design
locations throughout the world      % phrase drop "throughout the world"
e.g., as opposed to                 % phrase if you're giving examples, you're not talking about what isn't.  drop "e.g."
in addition, we also                % phrase remove either "also" or "in addition"
other related issues                % phrase probably remove "other"
the aforementioned                  % phrase "these xs" or "this x" would be less snooty
center around                       % phrase (cook) a center is a point: "center on" is okay.
could care less                     % phrase (cook) 'really? how much less could you care?' (should be couldn't)
grouped together                    % phrase redundant.  "grouped" alone should suffice.
put together                        % phrase long: "construct" "build" or "assemble"
consistent with each other          % phrase redundant.  "consistent" suffices.
be accomplished with                % phrase try "requires" "uses" "needs"?
the lack of knowledge of            % phrase would "X is unknown" work better?
gets to know                        % phrase you mean "learns"
trying to look like                 % phrase you mean "acting", "emulating", or "mimicing"
has got to be                       % phrase "must be"
got                                 % phrase try "became" "received" ?
gotten                              % phrase try "helped" ?
live in a vacuum                    % phrase a tired metaphor that makes me want to vomit.
positive impact                     % phrase try "benefit"
negative impact                     % phrase try "harm" or "consequences"
adverse impact                      % phrase try "harm" or "consequences"
adversely impacting                 % phrase try "harming" or "hurting"
discuss the issues of               % phrase could probably drop "the issues of" unless there's a list
the presence of                     % phrase not far from 'is', 'has', etc.
does not allow                      % phrase consider "forbids" or "prohibits"
and/or                              % phrase just say or.
there is the potential to           % phrase just say may.
there is the possibility that       % phrase just say might.
can be achieved                     % phrase maybe not so good?
find out                            % phrase perhaps determine?
in the absence of                   % phrase perhaps without?
in the presence of                  % phrase perhaps with?
set up                              % phrase perhaps create, configure, or initialize
in the face of                      % phrase can be overused.  try despite?
several times (at|of)               % phrase discouraged by Kurt.
a large degree of                   % phrase ick.
we start by first                   % phrase redundant. ("first, we" or "we start by").
in general, they are usually        % phrase redundant.
refers to the notion                % phrase define your term precisely if possible.
a significant amount of             % phrase probably just "significant"
real practical                      % phrase as opposed to imaginary practical?
people that are                     % phrase use people who are?
additional detail that we add       % phrase as opposed to additional detail that we subtract?
in some cases and not in others     % phrase "in some cases"
it is known that                    % phrase just say it.
caused due to                       % phrase "caused by"
a result of the fact that           % phrase "caused by"
results (indicate|show|suggest)     % phrase drop
research (indicates|show|suggest)   % phrase drop
can be attributed to the fact that  % phrase "is because"
a large set of                      % phrase probably don't care that it is a set.
a small set of                      % phrase probably don't care that it is a set: use 'a few'
provides a look at                  % phrase (timid) probably mean "shows".
in most cases                       % phrase "usually"
continue into the forseeable future % phrase "continue".
for the forseeable future           % phrase drop.
fail to successfully                % phrase "fail to" is sufficient.
Clearly,                            % syntax starting a sentence with clearly confuses me.
in different continents             % phrase ON different continents, IN different countries
(we|to) handle                      % phrase use a more specific verb like address, treat, solve
handling                            % phrase use a more specific verb like addressing, treating, solving, mitigating (unless handling errors or exceptions)
For the purposes of                 % phrase "For"
We observe that                     % phrase drop.
some degree of                      % phrase "some"
in the problem of                   % phrase (contributed by rap)
conclude several things             % phrase make (draw) several conclusions
extra bonus                         % phrase "bonus"
added bonus                         % phrase "bonus"
it is important to emphasize that   % phrase use diction to emphasize.
it is possible that                 % phrase "x may y"
caused due to                       % phrase "caused by"
recent work by                      % phrase could maybe be dropped, as the cite will include the date.
identify the location of            % phrase "find"
that go across                      % phrase "that cross"
ideally, we would like              % phrase "we would like"
enabling the ability to             % phrase "supporting" or "allowing" or "permitting"
absolutely essential                % phrase essential is.
we essentially do                   % phrase essentially is a poor adverb.  "The essence of our algorithm is a..."
Essentially,                        % phrase maybe "In essence," but could also be removed.
In this section (we|I)              % phrase "In this section, we", or "In this section, I"
essentially all                     % phrase "most"
past experience                     % phrase "experience" http://www.cmu.edu/styleguide/trickywords.html
particulary difficult primarily     % phrase simplify
intuition about why                 % phrase "intuition as to why"
Recall from above                   % phrase "recall"
Further, (I|we) will also           % phrase drop further or also
respectively                        % phrase unneeded.
in terms of                         % phrase don't need this.
the extent to which                 % phrase "how much"
make sure                           % phrase "ensure"
make up                             % phrase "constitute" "compose"
make use of                         % phrase "use"
make a decision                     % phrase "decide"
make a guess                        % phrase "guess"
since that time                     % phrase "since then"
choices to make                     % phrase "choices"
certain limitations                 % phrase what does 'certain' add to limitations?
will [a-z]* in the future           % phrase "will"
business entities                   % phrase "businesses"
rely primarily on                   % phrase "primarily" weakens "rely".  perhaps just "use" would be simpler.
has the potential to                % phrase can
have not yet developed              % phrase "have yet to develop"
to be effective,                    % phrase probably redundant.
provide information about           % phrase "tell how" "reveal" "expose" "disclose"
are different,                      % phrase "differ"
have already been                   % phrase "have been"? "were"?
as appropriate                      % phrase not needed?
only rarely                         % phrase "rarely" is probably enough.
is effective at                     % phrase "can"
foremost among them is              % phrase "foremost is" would be shorter.
those that have no                  % phrase those without
that have no                        % phrase "without"?
a variety of diverse                % phrase redundant
be highly valuable in               % phrase simplify.
the overall goal                    % phrase 'the goal'
sometimes an? [a-z]+ will           % phrase an x may
this is perhaps because             % phrase this may be because
adding an additional                % phrase redundant
IP protocol                         % phrase redundant
works well                          % phrase be more specific.
something                           % phrase could eliminate.
to keep from                        % phrase "to avoid"
[\.,] since (!then)                 % phrase probably you mean "because" unless you're talking about time. -- "has since" is okay.
performance characteristics         % phrase rare that characteristics adds.
takes into account                  % phrase considers
specify particular                  % phrase if specifying, particular should be redundant.
prototype implementation            % phrase "implementation" is redundant.
given a particular                  % phrase "given a" is probably enough
described in detail (in|below)      % phrase use "detailed"
relatively more                     % phrase more is already relative.
focus primarily on                  % phrase bad metaphor: subject of focus is singular.
primary focus                       % phrase bad metaphor: subject of focus is singular.
relatively more                     % phrase more is already relative.
gives [a-z]+ [a-z]+ information about % phrase use "tells" x
gives [a-z]+ information about      % phrase use "tells" x
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
have an effect on                   % phrase "affect"
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
we can see                          % phrase "we can see" isn't formal enough.
still remain                        % phrase "remain".
change over time                    % phrase "change"
turn into                           % phrase "become"
looking back in retrospect          % phrase pick.
ensures that there will be no       % phrase "prevents"
does have                           % phrase "has"
first step toward this              % phrase "toward this" can probably be dropped.
can potentially be                  % phrase "might be", or just "can be"
obviates the need for               % phrase just obviates x, not obviates the need for x.
it is indeed                        % phrase "it is", though still passive.
planning in advance                 % phrase when else might you plan?
a lot of                            % phrase "many"
keep in mind                        % phrase "consider" (or drop)
it is clear that                    % phrase if clear, you don't have to say it.
especially true                     % phrase true is an absolute, can't be especially true.
making it increasingly difficult    % phrase preventing, discouraging, impeding, blocking, slowing...
is potentially                      % phrase "may be"
have been [a-z]* in the past        % phrase 'in the past' is redundant with tense.
amount of time  % phrase "duration"
should ideally % phrase "should"
are of great benefit to % phrase "help" or "aid"
are of benefit to % phrase "help" or "aid" or "promote"
important here % phrase consider "relevant"
while at the same time % phrase "while" is enough.
are able to % phrase can
subvert the proper operation of % phrase subvert
speed slow % phrase speed is probably redundant.
of size no smaller than % phrase "of size" is probably redundant
of size no larger than % phrase "of size" is probably redundant
of size smaller than % phrase "of size" is probably redundant
of size larger than % phrase "of size" is probably redundant
might potentially % phrase "might"
in the context of % phrase "in" avoid, if possible.
increase the amount of % phrase probably just increase.
show the difference between % phrase compare
in addition, we also % phrase pick.
overhead efficiency % phrase huh?
have an effect on % phrase "affect"
have a signficant effect on %  phrase "affect"
we find % phrase can usually be removed
this suggests % phrase remove or make more precise
effective for providing	   	 % phrase remove
we performed a                   % phrase just use the verb directly
we perform a                     % phrase just use the verb directly
were able to                     % phrase could
are able to                      % phrase can


==> sections/archived/30-calibrate-qa.tex <==
In this section, we adapt the bucketing-based calibration framework designed for multi-class classification tasks on open-domain question answering, and we experiment temperature scaling on multiple QA benchmarks, both in- and out-of-domain. 
% State-of-the-art ODQA approaches follow the retrieve-and-read pipeline~\citep{chen2017reading}, 
% which we review in Section~\ref{subsec:base-model}, then we evaluate the temperature scaling approach over such ODQA pipeline on both in-domain and out-of-domain benchmarks in Section~\ref{subsec:base-calibration}.
%
%The most dominant approach for ODQA is to use a retrieve-and-read pipeline~\citep{chen2017reading}. 
%In this section, we first describe the open-domain QA model (Section~\ref{subsec:base-model})  that we use throughout this %paper, and then 
%we explore different implementations for calibrating the ODQA model (Section~\ref{subsec:base-calibration}).%
%methods on several QA datasets in order to find a reasonable calibration baseline for experiments in the later sections. 


% \chen{A possible concern is that we do not use DPR score, but rely on reader passage selection score. Maybe we can add a footnote to mention this and why we use this setting, so that reviewers will not complain again.}

\subsection{The ODQA Model}\label{subsec:base-model}
%We also briefly review the open-domain QA pipeline adopted in the experiments of this paper.
%We will use a DPR-BERT model trained on NQ for the experiments in the next few sections. 
% \sewon{Mostly wrote the reader part and skip retrieval, since the reader part is needed to explain the temperature scaling. If we use the score from DPR, we need to explain retrieval a bit more.}
% \chenglei{Yes the retrieval score is used so we probably need to add some brief description on the retriever part.}
We use the model from \citet{karpukhin2020dense}, which we call DPR-BERT. The model consists of both retrieval and reader components following the retrieve-and-read pipeline~\citep{chen2017reading}. 
%
The retrieval model is a dual encoder that computes the vector representation of the question and each Wikipedia passage, and returns the top-$K$ passages with the highest inner product scores between the question vector and the passage vector. 
The reader model is a BERT-based~\citep{devlin-19} span extraction model. It is given as input the concatenation of the question and each retrieved passage, and returns three logit values, representing the passage selection score, the start position score and the end position score respectively. These three logits are produced by three different classification heads on top of the final BERT representations. More precisely,
\begin{align*}
    \mathbf{H}_i &= \mathrm{BERT}(q,p_i) \in \mathbb{R}^{h \times L}, \\
    z^\mathrm{psg}(i) &= \left(\mathbf{H}_i\right)_{\texttt{[CLS]}}\mathbf{w}_\mathrm{psg} \in \mathbb{R}, \\ 
    z^{\mathrm{start}}(i, s) &= \left(\mathbf{H}_i\mathbf{w}^\mathrm{start}\right)_s \in \mathbb{R}, \\
    z^{\mathrm{end}}(i, e) &= \left(\mathbf{H}_i\mathbf{w}^\mathrm{end}\right)_e \in \mathbb{R},
\end{align*} where $\mathbf{w}_\mathrm{psg}, \mathbf{w}^\mathrm{start}, \mathbf{w}^\mathrm{end} \in \mathbb{R}^h$ are trainable parameters.

%At inference, there are two ways of scoring each span and making a prediction.

% \paragraph{Scoring of spans.}
% There are two ways of scoring spans.
% In {\em pipeline scoring}, we first choose the passage with the highest passage selection score $i_\mathrm{max} = \mathrm{argmax}_{1 \leq i \leq K}z^\mathrm{psg}(i)$ and then define a span score $S(s, e, i)$ as $$\left(z^{\mathrm{start}}(\hat{i}, s) + z^{\mathrm{end}}(\hat{i}, e)\right) \mathbb{I}[i=i_\mathrm{max}].$$ This is the method used in \citet{karpukhin2020dense}.
% We also explore an alternative {\em joint scoring}, where $S(s, e, i)$ is defined as $$z^{\mathrm{start}}(\hat{i}, s) + z^{\mathrm{end}}(\hat{i}, e) + z^\mathrm{psg}(i).$$

% The main difference is that it takes the passage selection logit $z^\mathrm{psg}$ into account.

% This is the method used in \sewon{TODO}.

% \paragraph{Answer Aggregation}
% We observe that in some cases there are multiple answer spans in the answer candidate set with the same surface form. Intuitively, the same answer string being predicted multiple times could imply that the model is more confident about that answer. To capture this effect, we explore an answer aggregation technique where we sum over the confidence scores of all occurrences of the answer string on the answer candidate set. 
%\sewon{I actually meant the `prediction' section of Section 3.1 discusses that.. since I thought this is less related to calibration but is more for the QA model itself. I'm OK with putting it here or editing the section above!}

\begin{comment}
\paragraph{Prediction.}
In the {\em no aggregation} method, we choose $\hat{s}, \hat{e}, \hat{i} = \mathrm{argmax}_{1 \leq s \leq e \leq L, 1 \leq i \leq K} S(s, e, i)$, and return the text span from the $\hat{s}$-th and the $\hat{e}$-th token of the $\hat{i}$-th passage as a prediction. This is the method used in \citet{karpukhin2020dense}.
In the {\em aggregation} method, we compute a score of each individual string by summing over their span scores, and return the string with the maximum score as a prediction. This is the method used in \sewon{TODO}.
\end{comment}



\subsection{Temperature Scaling For ODQA}\label{subsec:base-calibration}
%\sewon{This section is much clearer now, thank you for revising!!}

% Unlike classification problem, where the model directly outputs the probability of each class, in ODQA, the score of each candidate span relies on both passage and span scores. Therefore, as an approximation, 
To adapt temperature scaling on ODQA, we first compute the raw score for each candidate span, then apply softmax over the candidate set $\mathcal{C}$ to convert the raw span scores into probabilistic confidence values.
We explore two possible implementations:
%
%The main challenge in applying temperature scaling on ODQA is to first compute the confidence score of each answer prediction $y$: $\mathrm{Conf}(y)$.
%
%The main idea is to first compute a raw score for each candidate span, then apply softmax over the candidate set $\mathcal{C}$ to convert the raw scores into probabilistic distribution, and take the probability of the predicted span as the confidence score.
% Then we can apply temperature scaling to scale the raw score before taking the softmax as in ~\citet{guo2017calibration}.
%e need to assign a raw score to each candidate span. Upon these raw scores, we can apply softmax over the candidate set to convert the raw scores into probabilistic confidence. When computing the raw scores, we have explored several design choices and found that the best configuration is to sum up the passage selection logit, start position logit and end position logit as the raw score of each span. Taken together, this results in the following formulation for obtaining the confidence of each candidate prediction: 
%Nonetheless, unlike the classification problem as in \citet{guo2017calibration}, it is not trivial how to apply this approach to the open-domain QA model,
%Most prior work~\citep{guo2017calibration} evaluates temperature scaling on classification datasets only, and we are the first work to apply temperature scaling on extractive QA models with a retriever-reader pipeline.
%due to the much more complex pipeline.
% different possible scoring methods, and different possible aggregation methods.
\begin{comment}
In this paper, we explore three different design choices in adapting temperature scaling for ODQA: answer candidate generation, different possible scoring functions, and answer aggregation. 
Note that we describe each method assuming temperature scaling is used by using a hyperparameter $\tau$ that is tunable on the development data; the method without temperature scaling is equivalent to simply using $\tau=1$.
\end{comment}
%When applying temperature scaling on ODQA, we take the following adaptation.

% \sewon{I moved the candidate generation part as an implementation detail because I don't think it changes the high-level idea of the TS methods. Please feel free to put it back!}

% \chen{I think the following two sections can be largely shortened. For 3.2.1, we do not need to mention detailed parameters here, but \textbf{say why Joint and Pipeline has a difference}. And I suggest move 3.2.2 to experimental setup, while mention the ideas at the beginning of 3.2.}


% \paragraph{Answer Candidate Generation}
% We need to generate a set of top answer candidates so that we can apply softmax over the set to obtain a probabilistic distribution. We explore two possible ways of answer candidate generation:
% %
% % \sewon{@Chenglei does joint vs. pipeline here correspond to joint scoring and pipeline scoring in ``scoring of spans'' in Section 3.1? We might want to clarify this.}
% % \chen{I think these are two different concepts, but correct me if I'm wrong.}
% % \chen{edited above, but got confused ..}
% %


\paragraph{\textit{Joint Calibration}}
We perform inference on top $k=10$ retrieved passages for each question, and for each passage we obtain the top $n=10$ spans. This results in an answer set of $n \times k = 100$ spans per question. We score each candidate span as:

$$z^{\mathrm{start}}(\hat{i}, s) + z^{\mathrm{end}}(\hat{i}, e) + z^\mathrm{psg}(i).$$
%
After temperature scaling the confidence value is computed as:

\begin{small}$$\mathrm{Softmax}_{(i, s, e) \in \mathcal{C}}\left(\frac{z^\mathrm{psg}(i)+z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)}{\tau}\right).$$\end{small}


\paragraph{\textit{Pipeline Calibration}}
 We choose the passage with the highest passage selection score $i_\mathrm{max} = \mathrm{argmax}_{1 \leq i \leq K}z^\mathrm{psg}(i)$ and then define the span score $S(s, e, i)$ as $$\left(z^{\mathrm{start}}(\hat{i}, s) + z^{\mathrm{end}}(\hat{i}, e)\right) \mathbb{I}[i=i_\mathrm{max}].$$
%
In this case, we only keep the top $n=10$ spans from the top passage for each question. After temperature scaling, the confidence is computed as


$$\mathrm{Softmax}_{(i, s, e) \in \mathcal{C}}\left(\frac{z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)}{\tau}\right).$$

%We also explore other alternative model settings, since none of them outperforms the joint and pipeline calibration, we leave these experiments in the appendix.

% \subsubsection{Scoring Functions}

% There are several possible ways of computing a confidence value for each predicted answer span based on its passage selection logit, start logit, and end logit. Specifically, we consider the following four implementations as the confidence scoring functions:

% \paragraph{Joint S+E}
% We consider the raw score of the span as $z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)$, and compute $$\mathrm{Softmax}_{(i, s, e) \in \mathcal{C}}\left(\frac{z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)}{\tau}\right).$$

% \paragraph{Joint S+E+P}
% We consider the raw score of the span as $z^\mathrm{psg}(i)+z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)$, and compute \begin{small}$$\mathrm{Softmax}_{(i, s, e) \in \mathcal{C}}\left(\frac{z^\mathrm{psg}(i)+z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)}{\tau}\right).$$\end{small}

% \paragraph{Indep S+E}
% We compute the confidence score for the start and the end independently and multiply them. Specifically, we use
% \begin{small}$$\mathrm{Softmax}(\frac{z^{\mathrm{start}}(i, s)}{\tau_1} )
% \mathrm{Softmax} ( \frac{z^{\mathrm{end}}(i, e)}{\tau_2} ).$$\end{small}
% We use $\tau=\tau_1=\tau_2$ for simplicity.

% \paragraph{Indep S+E+P}
% Similar to above, we compute the confidence score for the start, the end, and the passage independently, and multiply over them.
% \begin{small}$$\mathrm{Softmax} ( \frac{z^{\mathrm{start}}(i, s)}{\tau_1} ) 
% \mathrm{Softmax} ( \frac{z^{\mathrm{end}}(i, e)}{\tau_2} )
% \mathrm{Softmax} ( \frac{z^{\mathrm{psg}}(i)}{\tau_3} ).$$\end{small}
% We use $\tau=\tau_1=\tau_2=\tau_3$ for simplicity.

% \vspace{.5em}
% \chenglei{Need to re-phrase this paragraph, it reads a bit confusing right now.}
% We find that it is generally better to match the scoring of spans for the prediction and for the confidence score. We thus report \textbf{Joint S+E} and \textbf{Indep S+E} for {\em pipeline scoring}, and \textbf{Joint S+E+P} and \textbf{Indep S+E+P} for {\em joint scoring}. Full results can be found in Appendix~\ref{}.



%\paragraph{Candidate Scoring} We need to assign a raw score to each candidate span. Upon these raw scores, we can apply softmax over the candidate set to convert the raw scores into probabilistic confidence. When computing the raw scores, we have explored several design choices and found that the best configuration is to sum up the passage selection logit, start position logit and end position logit as the raw score of each span. Taken together, this results in the following formulation for obtaining the confidence of each candidate prediction: 

%We conducted thorough comparison across different candidate generation and scoring configurations. We include the full results in the appendix.

%\chenglei{TODO: 1) Transfer the results from our other overleaf doc to the appendix here. 2) Add evaluations under the new metrics. }

\begin{comment}
\chenglei{Below is Sewon's original version, my proposal is to only mention the version that we end up using, and put the comparison with other alternatives in the appendix.}

\sewon{Not sure if we want to include all of them in the final version of the paper, but we can have a complete version first and decide what to exclude?}


\paragraph{Softmax.}
We follow \citet{jiang2021can} in casting the question answering problem as the multi-label classification problem by considering a set of possible answer spans as $\mathcal{C}$. Formally, $\mathrm{Conf}(x, \hat{y})$ is defined as $$\mathrm{Softmax}_{(i, s, e) \in \mathcal{C}}\left(\frac{z^\mathrm{psg}(i)+z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)}{\tau},\right)$$ where $\tau$ is a hyperparameter. 
Since enumerating over all possible spans of $K$ passages is expensive, we use the top-10 candidates as $\mathcal{C}$, where the top-10 answers are all from the best passage $\hat{i}$ and the top-10 spans are chosen based on $z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)$.\footnote{We explored taking the top-10 answers across different passages, but find it less competitive.\sewon{Wrote in this way, but is it true?}}
\sewon{
Looks like \citet{jiang2021can} used a different method to get the top-K spans (in page 3). Any idea how to explain it?
}

\paragraph{Softmax Independent.} TODO

\paragraph{Sigmoid.} Since we compute the confidence score given a particular prediction $\hat{y}$, we can consider it as a binary classification on whether or not $\hat{y}$ is correct. Formally, $\mathrm{Conf}(x, \hat{y})$ is defined as $$\mathrm{Sigmoid}\left(\frac{z^\mathrm{psg}(i)+z^{\mathrm{start}}(i, s)+z^{\mathrm{end}}(i, e)}{\tau}\right),$$where $\tau$ is a hyperparameter tuned on the development data.

\paragraph{Sigmoid Independent.} This method is similar to the sigmoid method but different temperature values are used for different logit values. Specifically, $\mathrm{Conf}(x, \hat{y})$ is defined as $$\mathrm{Sigmoid}\left(\frac{z^\mathrm{psg}(i)}{\tau^\mathrm{psg}}+\frac{z^{\mathrm{start}}(i, s)}{\tau^\mathrm{start}}+\frac{z^{\mathrm{end}}(i, e)}{\tau^\mathrm{end}}\right),$$where $\tau^\mathrm{psg},\tau^\mathrm{start},\tau^\mathrm{end}$ are hyperparameters. This may be effective because three logit values are often in different scales.

\sewon{I think at some point we also explored text-level aggregation where we marginalize over different spans with the same text expression. Do we want to talk about it here, or just skip?}
\end{comment}



%\sewon{Took from previous section 4}

%In this section, we evaluate and compare the calibration results under different calibration metrics. We will demonstrate that our new metrics are indeed more reliable than previous metrics and existing calibration techniques - both temperature scaling and training binary classifiers - work poorly for calibration under the new metrics.

% \chenglei{I think there should be a coherent logic flow to connect all the experiments and subsections in this section. Sewon \& Chen: please let me know if you have suggestions.}


\begin{comment}
\subsection{The ODQA Pipeline}

\sewon{Original version:}
When performing temperature scaling in open-domain question answering, we adopt a pipeline approach: we first select the best passage among the top 10 retrieved passages with the highest passage selection logit. From the top passage, we extract the top 10 spans with the highest (start logit + end logit). 

We score each predicted span by summing the raw passage selection logit, span start position logit and end position logit. We then perform a softmax over the top 10 predictions to obtain the probabilistic scores. We take the prediction with the highest probabilistic score as the final predicted answer and its probabilistic score is taken as the confidence for this prediction. 
\end{comment}

% \chen{Maybe mention in the table (an arrow?) that for ECE, ice, MacroCE, lower is better, for EM, higher is better}

\begin{table}[t]
\small
\begin{center}
\setlength{\tabcolsep}{1.4mm}{
\begin{tabular}{ l c @{\hspace{6\tabcolsep}} rrrc }
    %& \multicolumn{2}{c}{$\overbrace{\phantom{~~~~~}}^{\text{Section~\ref{sec:exp}}}$} & \multicolumn{2}{c}{$\overbrace{\phantom{~~~~~~~~}}^{\text{Section~\ref{sec:exp-new-metrics}}}$} \\
    && \multicolumn{2}{c}{Section~\ref{sec:calibrate_qa}} & \multicolumn{2}{c}{Section~\ref{sec:exp-new-metrics}} \\
 \toprule
    Model & TS & EM$_{\uparrow}$ & ECE$_{\downarrow}$ & ICE$_{\downarrow}$ & \metric{}$_{\downarrow}$ \\ 
 \midrule
    \multicolumn{5}{l}{\textbf{\em NQ}} \\
    Joint & -  & 32.9 & 27.1 & 47.8 &  43.6 \\
    Joint & \checkmark & 32.9 & 4.0 & \textbf{37.4} & \textbf{42.5} \\
    Pipeline & - & 34.1 & 48.2 & 55.1 & 44.2 \\
    Pipeline & \checkmark & 34.1 & \textbf{2.7} & 39.7 & 44.4 \\
 \midrule
    \multicolumn{5}{l}{\textbf{\em NQ $\rightarrow$ HotpotQA}} \\
    Joint & - & 24.9 & 41.0 & 54.7 & 45.7 \\
    Joint & \checkmark & 24.9 & 12.5 & 40.3 & \textbf{45.5} \\
    Pipeline & - & 22.6 & 59.6 & 65.9 & 47.4 \\
    Pipeline & \checkmark & 22.6 & \textbf{8.4} & \textbf{37.9} & 47.7 \\ 
 \midrule
    \multicolumn{5}{l}{\textbf{\em NQ $\rightarrow$ TriviaQA}} \\
    Joint & - & 33.6 & 25.4 & 48.6 & 45.1 \\
    Joint & \checkmark & 33.6 & 6.4 & \textbf{38.4} & 44.3 \\
    Pipeline & - & 34.2 & 48.2 & 54.5 & \textbf{43.7} \\
    Pipeline & \checkmark & 34.2 & \textbf{6.1} & 39.2 & 44.6 \\
    \midrule
    \multicolumn{5}{l}{\textbf{\em NQ $\rightarrow$ SQuAD}} \\
    Joint & - & 12.4 & 41.7 & 48.5 & 39.5 \\
    Joint & \checkmark & 12.4 & \textbf{12.4} & \textbf{26.6} & \textbf{39.7} \\
    Pipeline & - & 12.2 & 62.7 & 65.1 & 41.4 \\
    Pipeline & \checkmark & 12.2 & 13.5 & 29.1 & 43.9 \\
 \bottomrule
\end{tabular}}
 \caption{
    In-domain and OOD calibration results. \textit{Joint} and \textit{Pipeline} refer to whether the candidate set consists of top answer candidates from all top-10 retrieved passages or just the top-1 retrieved passage. All numbers are multiplied by 100 for better readability throughout the paper.
    EM: higher is better. Calibration errors: lower is better. Best calibration result in each group is in bold. Across all settings, temperature scaling significantly improves \abr{ece} but not \metric{}. 
    % \sewon{Proposal: No calibration vs Temp Scaling as a separate column?}
    % \chenglei{You mean turn this into a two-column wide table?}
    % \chen{I think this table is not clear, it's hard to readers to focus on the most important information. What Sewon suggested I think is to have another column related to temperature scaling, i.e., no calibration and temp scaling, so at least first column will be clearer. But i think it is not the highest priority for now, since we will also include generative QA here. }
    % \sewon{Q: Why is EM on SQUAD so bad? Any idea?} \chenglei{I think because DPR is bad at SQuAD retrieval.}
    % \sewon{yes that was my comment. I updated the table.}
 }
 \label{tab:temp_scale}
\end{center}
\end{table}


\subsection{Experiments}\label{subsec:base-exp-setup}

%\chenglei{Will also put some other implementation details here.}
%We introduce the QA datasets that we will be using is this paper: NQ, SQuAD, TriviaQA, HotpotQA. 

We experiment the above temperature scaling method 
on both in-domain and OOD settings, since \citet{Desai2020CalibrationOP,jiang2021can} mentioned that OOD calibration is more challenging than in-domain calibration.
%We use four QA datasets: \textbf{Natural Questions (NQ)}~\citep{kwiatkowski-19}, \textbf{SQuAD}~\citep{rajpurkar-16}, \textbf{TriviaQA}~\citep{joshi-17} and \textbf{HotpotQA}~\citep{yang2018hotpotqa}.\footnote{We include dataset details in appendix.}
We use \textbf{Natural Questions (NQ)}~\citep{kwiatkowski-19} as the in-domain dataset, and \textbf{SQuAD}~\citep{rajpurkar-16}, \textbf{TriviaQA}~\citep{joshi-17} and \textbf{HotpotQA}~\citep{yang2018hotpotqa} as the out-of-domain datasets.\footnote{We include dataset details in appendix.}
%
%\sewon{I think I wrote these dataset descriptions, but now think we can cut them if we need to save space, since we aren't looking into details of each dataset anyways.}
%
%
All hyperparameters are tuned based on the in-domain development data (NQ development data).
%For temperature scaling, we tune the temperature scalar on the NQ development set, evaluate on NQ test set (in-domain) and three other QA datasets (OOD).
We report exact match (EM) score for answer accuracy %(note that temperature scaling does not impact the EM score),
and ECE for calibration results. 
%Note that temperature scaling does not impact the EM score.


% \paragraph{Implementation details.}
% We follow \citet{karpukhin2020dense} in using the plain text portion of the English Wikipedia dump from 12/20/2018. We use $K=10$.

%\paragraph{Candidate Generation}
% When computing the candidate set $\mathcal{C}$, enumerating over all possible spans of $K$ passages is expensive. We therefore approximate $\mathcal{C}$ by taking the top 10 predictions from each of $K$ passage, resulting in $|\mathcal{C}|=100$ with $K=10$.

%We first obtain a list of candidate answers for each question. We explored two possibilities: 1) We keep the top 10 predictions from each of top 10 retrieved passages. This results in a total of 100 candidate predictions per question. We name this approach \textit{joint} calibration. 2) We only choose from the top 10 predictions from the passage with the highest passage selection score. This results in a candidate pool of size 10 instead of 100. We name this approach \textit{pipeline} calibration.  By default we use the pipeline approach as we found it to produce slightly better calibration results.

% \subsection{Results}


% \subsection{Results}\label{subsec:base-results}

% \chenglei{Will also add tables for the OOD datasets. Will re-write this section after I fill in these tables.}

According to Table~\ref{tab:temp_scale}, we observe that without calibration, both joint and pipeline approaches have high ECE scores, and the pipeline approach incurs higher out-of-the-box calibration error.
Applying temperature scaling significantly lowers ECE in all cases, including both in-domain and OOD settings. 
As expected, OOD settings incur higher ECE than the in-domain setting even after calibration. 
However, in the next section, we challenge this ``success'' by re-examining the bucketing mechanism in ECE computation. 

% \sewon{Is there anything we want to talk about RE joint vs. pipeline?}

% \paragraph{Joint TS also improves ECE out-of-distribution.} \sewon{TODO}

% \subsection{Analyses}\label{subsec:base-analysis}
% \sewon{TODO: describe the issues with ECE}


==> sections/archived/40-metrics.tex <==
%In the previous section, we showed that adapting temperature scaling on ODQA improves ECE significantly. However, in this section, we challenge this success by re-examining the bucketing mechanism in ECE computation. 
%
% Despite current approaches work well, we find the evaluate metric, ECE, has major flaws.
%the popularity of ECE (in particular the interval-based ECE) as the calibration metric, we find major flaws of ECE.
In this section, we use case studies to illustrate the flaws of \abr{ece}, provide complementary views of calibration and correspondingly propose new calibration metrics.
\sewon{I think this section can overall be more concise. I can take a pass once the figure is ready.}

\chen{Do we want to use \abr{ece} or ECE? let's be consistent.}


% \chen{Do you think there are some duplicates in 4.1 and 4.2?}

\subsection{What's Wrong With ECE?}

% \chen{What about something like Gap between ECE and real calibration setting?}

% In this section, we use some illustrative examples to demonstrate the flaws of the ECE metric. In particular, we show that low ECE does not necessarily correspond to good calibration performance due to the bucketing mechanism. 

We begin with a case study on \abr{ood} setting where we train a DPR-BERT model on NQ and evaluate on HotpotQA.\footnote{We illustrate the problem with a case study on HotpotQA, the same issues hold true on other \abr{ood} datasets as well.} According to Figure~\ref{fig:ece_illustration},
we observe that the uncalibrated model is over-confident as the confidence is higher than the accuracy for all buckets. After temperature scaling, the accuracy and confidence are close, resulting in a significant \abr{ece} reduction. 
%
However, we argue the result misleadingly over-estimated the effectiveness of temperature scaling for the following reasons:\footnote{Our findings apply to both equal-width and equal-mass binning of \abr{ece}, although we use equal-width binning for illustration.\chen{why?}}



%  \begin{figure}[t]
% \centering
% \includegraphics[width=0.50\textwidth]{figures/hotpotqa_uncalibrated.png}
% \caption{Uncalibrated results on HotpotQA. x-axis: confidence ranges of buckets. Solid line: average accuracy of each bucket. Dashed line: average confidence of each bucket. Histogram: relative sizes ($\%$) of each bucket.
% \sewon{Proposal: let's explicitly put the axis title? I think it'll be obvious for people familiar with calibration, but won't be obvious for others.}
% \sewon{Proposal: Combine Fig 2 and 3, have figures for NQ as well, so that there is one 2-column figure with four small subfigures? IMHO this is the most important figure in this paper.}
% \chen{I agree with Sewon's proposal, those four figures will look better, also could save some space. }
% }
% \label{fig:hotpotqa_uncalibrated}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.50\textwidth]{figures/hotpotqa_ts.png}
% \caption{Results on HotpotQA after temperature scaling. x-axis: confidence ranges of buckets. Solid line: average accuracy of each bucket. Dashed line: average confidence of each bucket. Histogram: relative sizes ($\%$) of each bucket.}
% \label{fig:hotpotqa_ts}
% \end{figure}


 \begin{figure*}[t]
 \centering
 \includegraphics[trim=3.1cm 0.2cm 3.1cm 0.2cm,clip=true,width=\linewidth]{figures/calibrate_fig2.png}
%  \includegraphics[width=1.2\textwidth]{figures/calibrate_fig2.png}
\caption{Bucketing distribution of predictions on NQ (in-domain) and HotpotQA (\abr{ood}). We show both uncalibrated (before TS) and calibrated (after TS) results. In all plots, x-axis represents the average confidence of each bucket, y-axis represents the average answer accuracy for the dashed line plot and represents the relative bucket sizes for the histogram plot.}
\label{fig:ece_illustration}
 \end{figure*}


%Before any post-hoc calibration, the model's predictions are bucketed as in Figure~\ref{fig:hotpotqa_uncalibrated}.

% Acc:  [-1.0, 0.0, 0.05, 0.08, 0.11, 0.18, 0.23, 0.2, 0.2, 0.27]

% Conf:  [-1.0, 0.19, 0.27, 0.36, 0.46, 0.55, 0.65, 0.75, 0.85, 0.98]

% Sizes:  [0, 1, 20, 95, 201, 276, 353, 381, 453, 1767]

% interval-based ECE:  59.60

%We can observe that the uncalibrated model is over-confident on this OOD test set as the confidence is much higher than the accuracy for all buckets.

%We then perform temperature scaling on this model. We use a temperature scalar 9.54 as tuned on the HotpotQA dev set. 
%It is expected that the temperature scalar is large since the original predictions are over-confident.
%After we apply temperature scaling with this temperature scalar, we plot the prediction bucketing in Figure~\ref{fig:hotpotqa_ts}. 


% Acc:  [-1.0, 0.16, 0.26, 0.34, 0.34, 1.0, -1.0, -1.0, -1.0, -1.0]

% Conf:  [-1.0, 0.17, 0.24, 0.34, 0.42, 0.51, -1.0, -1.0, -1.0, -1.0]

% Sizes:  [0, 1521, 1633, 357, 35, 1, 0, 0, 0, 0]

% interval-based ECE:  0.95

%We outline the reasons why such calibration result is not ideal and how the interval-based ECE is misleading:
\noindent
1) \textbf{Most instances are assigned similar confidence.}
%\sewon{-> Most instances assigned to 1--2 bins?}
After calibration, all predictions have low confidence (which match the relatively low accuracy). This is essentially conveying the message that all predictions are not confident, even for correct ones. 
% Such calibrated predictions therefore do not allow users to identify correct predictions.  
% We argue that the low ECE under such case has little practical implication because it is not telling the difference between correct and wrong predictions.
An ideal calibration metric should penalize such scenario and encourage the calibrator to differentiate  correct and wrong predictions by assigning high and low confidence scores respectively. 

\noindent
2) \textbf{Bucketing causes cancellation effects, thus underestimating the true calibration error.} A large number of predictions are clustered in the same buckets (in the [0.1, 0.4] range in Figure~\ref{fig:ece_illustration}). As a result, there exists many over-confident and under-confident predictions in the same bucket, causing a cancellation effect  where over- and under-confidence values are averaged to become closer to the average accuracy.
%However, on the instance level, over- and under-confidence still exists for wrong and correct predictions. 
% For instance, when we evaluate the same temperature value on the subset where the question has no correct prediction (where the models tends to be overconfident), the ECE is 21.58; and when we evaluate on the subset where the question has multiple correct predictions (where the model tends to be underconfident), the ECE is 21.03.\chen{This example seems unnecessary to me} Both numbers are much larger than the ECE on the entire test set, illustrating the issue that the cancellation effect gives a misleadingly low ECE result. 
A better calibration metric should avoid such cancellation effects caused by bucketing.


%We include more such examples on different test sets including both IID and OOD evaluations in the appendix. We find that these problems persist across all settings and the conventional interval-based ECE metric fails to reflect these issues. 

\subsection{The Alternative View of Calibration}
% \sewon{I love the intuition in this section. Maybe we can consider merging it with Section 2.4?}
% \chen{Agree}

The dominant calibration framework as evaluated by ECE follows an expectation point of view: the goal is for the confidence to match the expected accuracy.
%
However, this goal can be trivially achieved by simply outputting the similar confidence for all predictions that match the expected accuracy, as in the case of temperature scaling. 
%
In practical settings, such calibration results are not particularly useful because users cannot differentiate correct and wrong predictions based on such clustered confidence values. 
Hence, we propose the alternative view of calibration where the goal is to \textbf{differentiate between correct and wrong predictions}. 
We argue that achieving this goal would bring better practical values for real use cases of calibration. 
Towards this end, we propose a new calibration metric that aligns closely with our objective. 

% \sewon{Possible Q: this mainly explains equal-width binning. Why is equal-mass binning not good either?}
% \chen{Interesting, I did not see equal-mass binning mentioned in this section (but agree readers may have this question), what about we add a footnote explaining this problem?}
% \chenglei{I said at the end of 2.1 that equal-width and equal-mass have very similar trends which I think would account for this - same problems here apply for equal-mass as well.}


\subsection{New Metric: \metric{}}
%
%
%  In Section~\ref{sec:re-eval}, we compare them with the ECE metric on several QA datasets and various calibration methods, and find that the temperature scaling method, which has been shown to be highly effective in a range of prior work, is in fact ineffective.
% In Section~\ref{sec:related}, we make the connection between our metrics and other metrics proposed in prior work. \sewon{I think we can write in the way that, there have been metrics proposed earlier to migrate issues with ECE, but we use the metrics that are {\em minimal} modification to ECE given that ECE is the most widely used metric. Not exactly sure how to make this clear...}
% \chenglei{I re-write this section.}
%In this section, we introduce our new proposed calibration metrics ICE and CCE. We compare them with previous previous ECE metrics on several QA datasets to illustrate the advantages of our new metrics. Moreover, we show that the temperature scaling method is not effective in improving calibration - contrary to what previous works conclude. 

One straightforward solution to avoid the cancellation effect is to remove bucketing and accumulates the calibrator error of each individual prediction. 
We refer this metric, which is the base of our proposed metric, as
\textbf{Instance-level Calibration Error (ICE)}:\footnote{Note that this is also equivalent to ECE with equal-mass binning under the condition that $M=N$ (i.e., the bucket size is always 1). 
} 
%\sewon{Proposal: hint first that the MacroCE is the main metric? People might be confusing because the title says MacroCE and now we are introducing ICE.}

$$\mathrm{ICE} = \frac{1}{n}\sum^{n}_{i=1} |\mathbb{I}(y_i=\tilde{y}_i) - \mathrm{Conf}(x_i, \tilde{y}_i)|.$$
%

However, 
% as we will show in the next section, 
the ICE metric has another important flaw: it is highly sensitive to the model accuracy. 
% \sewon{Cite the vision paper that claims it shouldn't be sensitive to accuracy?} 
For instance, if most predictions are correct,  applying a small temperature scalar to boost all confidence scores lowers the ICE score, but not penalizing the wrong predictions with high confidence scores, as the small proportion of wrong predictions would not contribute much to the overall metric. 


To overcome this issue, we propose to take equal consideration of both correct and wrong predictions with the \textbf{Macro-average Calibration Error (\metric)}: 
%\sewon{delete category? I have been thinking what category means was never clear.}
% \todo{Fix the following eqs, too many space, use align}

% \begin{align*}
%     \mathrm{Acc}(B_m)&=\frac{1}{|B_m|}\sum_{i=1}^{|B_m|}\mathbb{I}(y=\hat{y}), \\
%     \mathrm{Conf}(B_m)&=\frac{1}{|B_m|}\sum_{i=1}^{|B_m|}\mathrm{Conf}(x, \hat{y}), \\
%     \mathrm{ECE}&=\sum^{M}_{m=1} \frac{|B_m|}{N} |\mathrm{Acc}(B_m) - \mathrm{Conf}(B_m)|,
% \end{align*}

\begin{align*}
\mathrm{ICE_{pos}} &= \frac{1}{p} \sum^{p}_{i=1} (1 - \mathrm{Conf}(x_i, \tilde{y}_i)), \forall \tilde{y}_i = y_i,\\
\mathrm{ICE_{neg}} &= \frac{1}{n} \sum^{n}_{i=1} ( \mathrm{Conf}(x_i, \tilde{y}_i) - 0), \forall \tilde{y}_i \neq y_i,\\
\mathrm{MacroCE} &= \frac{1}{2} (\mathrm{ICE_{pos}} + \mathrm{ICE_{neg}}).
\end{align*}


%In this way, $\mathrm{MacroCE}$ gives equal weight to positive (correct) and negative (wrong) predictions. We will demonstrate the advantage of %doing so in the next section. 

% \chen{I suggest we make three figures on section 4.4}

We conduct the same experiment as Section~\ref{sec:calibrate_qa}, evaluated by ICE and MacroCE. According to Table~\ref{tab:temp_scale} (rightmost two columns), we find that temperature scaling improves on ICE metric, and such improvement is more significant with lower EM (NQ $\rightarrow$ SQuAD). Since most predictions are incorrect, applying a high temperature scalar results in lower ICE score. Our proposed metric, \metric{}, is not sensitive to model accuracy, and as a result, we find applying temperature scaling has no improvement on 
\metric{}.
%we find the stark contrast that while temperature scaling brings significant improvement on ECE and ICE, it has no improvement on MacroCE. 
%Moreover, different metrics ranks different calibration methods differently, for example, for in-domain calibration, joint calibration gets worse ECE but better MacroCE over pipeline calibration.
\sewon{Expand it more? Feel like this is an important discussion and ends really fast lol.}
\chen{I added some take-aways, but guess we could add a few more.}

In the following subsection, we provide a series of controlled experiments to highlight why MacroCE is more informative. 


\subsection{Comparing Different Metrics Through Controlled Experiments}

We design three controlled experiments (NQ in-domain evaluation) to compare \abr{ece} and \metric. 
%These results would illustrate why MacroCE provides a better account oscf the actual calibration results. 

% For temperature scaling, we perform three sets of experiments for a thorough analysis on how TS works and use the results as a lens to better understand what different metrics capture.

\paragraph{Temperature Scaling with Different Temperature Scalars}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/all_temperatures.png}
    \caption{Calibration errors after temperature scaling. x-axis represents different temperature values; lines with different colors represent different metrics. MacroCE stays relatively constant while ECE varies largely at different temperature values.}
    \label{fig:all_temperatures}
\end{figure}

\sewon{I think I would cut this paragraph if we are over 8 pages.}
\chen{Agree, let's leave it here first.}

% \chenglei{Will try to make plots look nicer later. It should be clear even without colors. Also: unify the naming of different metrics.}

%vary the temperature scalar $\tau$ from 0.01 to 10.0 with a 0.01 interval and 
We apply temperature scaling with varying temperature scalar $\tau$.
% This offers a direct comparison between these metrics and also allow us to understand the impact of temperature scaling. 
% The model accuracy (EM) stays at 34.18. %
According to Figure~\ref{fig:all_temperatures},
as we increase the temperature value, the confidence scores decrease, and consequently ICE$_{\mathrm{pos}}$ increases and ICE$_{\mathrm{neg}}$ decreases. Meanwhile, MacroCE stays constant while ECE changes drastically, which reflects the flaw of temperature scaling: a single temperature value cannot improve calibration for both correct and wrong predictions simultaneously. Such flaw is only captured by MacroCE. 



\begin{table}[t]
\small
\begin{center}
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{ l c c c c }
 \toprule
  & Temp & ECE & ICE & MacroCE \\ 
 \midrule
    \multicolumn{5}{l}{\textbf{\em Acc=10\%}} \\
    Before Calibration & 1.00 & 69.97 & 71.93 &  44.32 \\
    After Temp Scaling & 10.00 & 11.49 & 26.08 & 46.90 \\
 \midrule
    \multicolumn{5}{l}{\textbf{\em Acc=50\%}} \\
    Before Calibration & 1.00 & 34.15 & 44.50 & 44.50 \\
    After Temp Scaling & 4.27 & 5.60 & 42.42 & 42.42 \\
 \midrule
    \multicolumn{5}{l}{\textbf{\em Acc=90\%}} \\
    Before Calibration & 1.00 & 7.96 & 8.08 & 45.33 \\
    After Temp Scaling & 0.47 & 9.08 & 13.18 & 47.77 \\
 \bottomrule
\end{tabular}}
 \caption{Calibration results where we re-sample the predictions to control the model accuracy (10\%, 50\%, 90\%; same for both dev and test sets). We also report the tuned temperature values along with the calibration results under different metrics.}
 \label{tab:analysis2}
\end{center}
\end{table}


\paragraph{Temperature Scaling at Different Accuracy Levels}

% \chen{Section 5.1 and 5.2 could be two analysis in our new proposed section 4, each has a short paragraph;}
% \chenglei{I plan to insert a set of plots here. The y-axis is the calibration error (each line represents one metric), the x-axis is the accuracy.} \sewon{Sounds great to me! I think we want to report the accuracy (regular accuracy metric) as well, probably in the separate table or graph in the earlier section.}

\begin{comment}
\chenglei{Raw results below, will turn into a plot or table later (@Sewon: feel free to create a placeholder table here, I'll put the results in later). For full results, refer to the google doc starting from page 46.}

accuracy = 10\%

Before Calibration:

interval-based ECE:  69.97


ICE: 71.93

CICE: 44.32

After Calibration (temperature = 10):

interval ECE: 

Acc:  [-1.0, 0.05, 0.1, 0.26, 0.39, -1.0, -1.0, -1.0, -1.0, -1.0]

Conf:  [-1.0, 0.16, 0.24, 0.34, 0.42, -1.0, -1.0, -1.0, -1.0, -1.0]

Sizes:  [0, 511, 354, 117, 18, 0, 0, 0, 0, 0]

test ECE:  11.49

ICE: 26.08

CICE: 46.90


accuracy = 50\%

Before Calibration:

interval-based ECE:  34.15

ICE: 44.50

CICE: 44.50

After Calibration (temperature = 4.27):

interval ECE

Acc:  [-1.0, 0.26, 0.27, 0.37, 0.54, 0.64, 0.7, 0.71, 0.73, 0.92]

Conf:  [-1.0, 0.17, 0.25, 0.35, 0.45, 0.55, 0.65, 0.75, 0.85, 0.92]

Sizes:  [0, 65, 193, 192, 155, 106, 106, 95, 75, 13]

test ECE:  5.599602523790778


ICE: 42.42

CICE: 42.42


accuracy = 90\%

Before Calibration:

interval-based ECE: 7.96

ICE: 8.08

CICE: 45.33


After Calibration (temperature = 0.47):

interval ECE

Acc:  [-1.0, -1.0, -1.0, 0.75, 0.86, 0.77, 0.89, 0.81, 0.84, 0.91]

Conf:  [-1.0, -1.0, -1.0, 0.37, 0.46, 0.55, 0.64, 0.75, 0.85, 0.99]

Sizes:  [0, 0, 0, 4, 7, 26, 35, 31, 37, 860]

test ECE:  9.07731574614255


ICE: 13.18

CICE: 47.77

\end{comment}

%re-sample the dev and test set of NQ to
We re-sample the data to control the model accuracy, and examine the effect of temperature scaling at different accuracy levels. 
% An ideal metric should not be sensitive to the model accuracy. 
%
According to Table~\ref{tab:analysis2}, before calbration, the ECE score decreases with higher model model accuracy, since 
%This is not because models are becoming better calibrated (since we are using the same model checkpoint), but rather, the 
higher accuracy matches the over-confidence predictions and gets rewarded by low ECE score. Such finding also applies to ICE, 
since the majority of predictions are correct, the impact of negative predictions with over-confidence is marginal.
%metric  is correct predictions at $90\%$ accuracy. 
%as well. As a high accuracy ($90\%$), the high confidence matches the high accuracy. 
%However, the negative predictions have over-confidence but their impact is marginal to the overall ICE metric since the majority is correct predictions at $90\%$ accuracy. 
MacroCE results remain stable across all accuracy levels. As model accuracy increases, ICE$_{\mathrm{pos}}$ decreases and ICE$_{\mathrm{neg}}$ increases. MacroCE captures the trade-off and implies the model remains poorly calibrated.
% since it is not becoming better at differentiating correct and wrong predictions. 


% 1) At extreme accuracy levels, the clustering in a few bucket problem is more extreme. The only case where the bucket size is spread out is at the accuracy = 50\% case. 


% 2) For interval-based ECE, the error before calibration keeps decreasing as the model accuracy increases. This is not because models are becoming better calibrated (since we are using the same model checkpoint), but rather, the higher accuracy matches the over-confidence. This highlights the flaw of interval-based ECE.

% 3) Similar case for ICE: you can see that the uncalibrated ICE keeps decreasing as model accuracy increases, this is also because the over-confidence and high accuracy matches and so the gap is smaller.

% 4) On the contrary, the MacroCE results remain stable across all accuracy levels. As model accuracy increases, ICE-pos decreases while ICE-neg increases. The average MacroCE captures such trade-off and reflects that the model remains poorly calibrated since it is not becoming better at differentiating correct and wrong predictions. 



\begin{table}[t]
\small
\begin{center}
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{ l c c c c }
 \toprule
  & Temp & ECE & ICE & MacroCE \\ 
 \midrule
    \multicolumn{5}{l}{\textbf{\em Development=90\% $\rightarrow$ Test=10\%}} \\
    Development & 0.47 & 7.20 & 12.29 & 46.64 \\
    Test & 0.47 & 80.54 & 81.49 & 47.39 \\
 \midrule
    \multicolumn{5}{l}{\textbf{\em Development=10\% $\rightarrow$ Test=90\%}} \\
    Development & 10.00 & 12.23 & 26.88 & 47.48 \\
    Test & 10.00 & 63.87 & 68.00 & 46.94 \\
 \bottomrule
\end{tabular}}
 \caption{Calibration results under subpopulation shift. In the first case, we tune the temperature value on a development set with only 10\% correct predictions but evaluate on a test set with 90\% correct predictions. We reverse the setup in the second case. Temperature scaling fails under such settings. ECE misleadingly tells that the models is well calibrated on the development set while MacroCE stays poor on both development and test sets.}
 \label{tab:analysis3}
\end{center}
\end{table}

\chen{I think we should combine table 2 and 3 into one table.}

\paragraph{Temperature Scaling under Subpopulation Shift}

We consider the subpopulation shift setting, where the development and test set accuracy differs largely. 
%
In particular, we consider the cases where we: 1) tune temperature on a development set with 90\% accuracy and evaluate on a test set with 10\% accuracy; and 2) tune temperature on a development set with 10\% accuracy and evaluate on a test set with 90\% accuracy.
%All data are re-sampled from the NQ dev and test set. 
%
According to Table~\ref{tab:analysis3}, we observe that ECE and ICE are sensitive to the model accuracy but not MacroCE. Temperature scaling selects a low temperature on the highly accurate development set which does not transfer to the test set with low accuracy, which indicates that temperature tuning does not hold against subpopulation shift.
% 
MacroCE reflects the poor calibration of the model on both cases, insensitive to the subpopulation shift.

All three experiments indicate that MacroCE is a more reliable calibration evaluation metric. 
We thus prioritize MacroCE evaluation throughout the rest of the paper.
% In the next section, we examine whether other calibration techniques besides temperature scaling are effective in improving MacroCE.




\begin{comment}
\chenglei{Raw results below, will turn into a table or plot later. Again feel free to first create a placeholder table here and I will fill in the corresponding results. }

Results:

Case 1:

Dev Set 90\% Accuracy:

temp 0.47,

interval ECE: 7.20

density ECE: 7.46

ICE: 12.29

CCE: 46.64

Test Set 10\% Accuracy:

interval ECE: 80.54

density ECE: 80.54

ICE: 81.49

CICE: 47.39


Case 2:

Dev Set 10\% Accuracy:

temp 10.0

interval ECE: 12.23

density ECE: 12.23

ICE: 26.88

CICE: 47.48

Test Set 90\% Accuracy:

interval ECE: 63.87

density ECE: 63.87

ICE: 68.00

CICE: 46.94
\end{comment}




==> sections/archived/50-prev-methods.tex <==
Given the above criticisms against ECE and the conclusion that temperature scaling does not help MacroCE, we examine several other calibration methods to see if they are effective under MacroCE. These methods include: feature-based classifier, neural reranker, and label smoothing. 
% We will show that different metrics give different conclusions about these calibration methods and under the MacroCE metric, none of these methods works well. 
All experiments are conducted on NQ in-domain data. 

\sewon{Proposal: right now each subsection has each method + result for that method. What about describing all methods, and then describe all results? This seems to make more sense because our table is also made in this way. Also, for each method, we can only briefly describe and move details into Appendix.}
\sewon{Another proposal: we could possibly merge Section 5 and 6? Because I think the baselines for the new calibration method in Section 6 should be the methods in Section 5, so it might be good to merge the table and discuss them altogether.}

\subsection{Feature Based Classifier}

\begin{table}[t]
\small
\begin{center}
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{ c c c c c }
\toprule
  & EM & ICE$_{\mathrm{pos}}$ & ICE$_{\mathrm{neg}}$  & MacroCE \\ 
  \midrule
  No Calibration & 32.85 & 31.46 & 55.74 & 43.60 \\
  \midrule
  \multicolumn{5}{l}{\textbf{\em Feature-based Classifier}} \\
%   Lin Regression & 35.26 & 7.90 & 79.56 & 43.73 \\
 LR & 35.10 & 3.84 & 88.54 & 46.19 \\  
 SVM & 34.29 & 4.88 & 87.20 & 46.04  \\
 kNN & 34.29 & 0.47 & 97.46 & 48.97 \\
 Random Forest & 34.43 & 7.56 & 84.04 & 45.80 \\
 MLP & 35.68 & 3.03 & 90.78 & 46.91 \\
 \midrule
\multicolumn{5}{l}{\textbf{\em Neural Reranker (ReConsider)}} \\
 Softmax  & 35.62 & 60.19 & 39.20 & 49.69 \\
 Sigmoid  & 35.62 & 9.37 & 72.59 & 40.97 \\
 \midrule
    \multicolumn{5}{l}{\textbf{\em Label Smoothing}} \\
    LS  & 35.76  & 32.08 & 56.04 & 44.06 \\
    LS + TS  & 35.76 & 55.72 & 29.52 & 42.62 \\
 \bottomrule
\end{tabular}}
 \caption{
We evaluate several types of calibration methods. Firstly, 
we train binary classifiers  as the calibrator. 
%  We report both the question answering EM score and the category-average calibration error on the test set. 
 The classifiers include logistic regression (LR), SVM, kNN, random forest, and multilayer perceptron (MLP). 
%  We also include a linear regression baseline where we cast the calibration task as regression rather than classification and minimize the mean squared error. 
%  Using a feature-based calibrator improves answer selection as shown by the higher EM score, but they are over-confident and cause high calibration errors on negative predictions, and therefore no improvement on MacroCE.
Secondly, we train a neural answer reranker and explore using  softmax and sigmoid to convert the raw reranker logits to confidence values. Lastly, we re-train the DPR-BERT model with label smoothing (LS) and we also try applying temperature scaling on top of the model trained with label smothing (TS + LS). 
All these methods can improve the QA performance (EM), but there is little improvement on MacroCE. 
 }
 \label{tab:classifiers}
\end{center}
\end{table}



One widely-used calibration method is to train a feature-based classifier to predict the correctness of predictions~\cite{Kamath2020SelectiveQA,Zhang2021KnowingMA,Ye2022CanEB}. 
In our experiments, 
%We experiment with feature-based classifiers where we identify a set of potentially relevant features for question answering, and then train a classifier on these features. 
 %
we include the following features based on previous work and domain knowledge~\cite{Kamath2020SelectiveQA,Rodriguez2019QuizbowlTC}: 
the length of the question, passage and predicted answer; raw and softmax logits of passage, span start and end selection; softmax logits of other predicted answers among the top 100 answer candidates; the number of times that the predicted answer appears in the passage and the question; the number of times the predicted answer appears in the top 100 predictions; and the difference between the current and the next most confident prediction.
%
To train the classifier, we use the QA model's predictions on the NQ dev set as the training data. 
%For each NQ dev question, we consider the top 10 retrieved passages and for each passage we consider the top 10 predicted answers. This results in 100 predictions per question.
%When training the classifier, we down-sample the wrong predictions to create a balanced training set.
We hold out 10\% predictions as the validation set and we apply early stopping based on the validation loss. 
%This results in a training set of size 38K and a dev set of size 4.2K. 
During inference, we directly use the predicted probability as the confidence value.
%
% We include the following set of features for training the classifiers: 
% the length of the question, passage and predicted answer; raw logits and softmax logits of passage selection, span start selection and span end selection; softmax logits of other predicted answers among the top 100 answer candidates; the number of times that the predicted answer appears in the passage and the question; the number of times the predicted answer appears in the top 100 predictions; and the difference between the prediction and the next most confident prediction (both in terms of raw scores and softmax logits).
%
We train multiple binary classifiers with these features and compare the calibration performance on the NQ test set.

According to Table~\ref{tab:classifiers},
% We also include the interval-bucket confidence distribution of each classifier and the interval-based ECE evaluations in the appendix.
%
all classifiers improve the EM score due to better answer reranking, however they suffer from over-confidence as shown by the large calibrator error on negative predictions (ICE$_{\mathrm{neg}}$), and as a result, there is no improvement on MacroCE.
We conclude that the feature-based classification approach does not work well for calibration as it still assigns high confidence for negative predictions.
%

%Additionally, we take a look at the trained logistic regression model to understand what features have higher importance. The features with the highest weight magnitude are: the number of times the prediction occurs in the top 100 predictions; the number of times the prediction occurs in the question; passage and span selection logits.


% \begin{table*}
% % \small
% \begin{center}
% \setlength{\tabcolsep}{5mm}{
% \begin{tabular}{ c c c c c }
% \toprule
%   & EM & CCE-pos & CCE-neg & CCE-avg \\ 
%   \midrule
%  No Calibration$_{c=10}$ & 34.07 & 10.11 & 78.30 & 44.21 \\
%   No Calibration$_{c=100}$ & 32.85 & 31.46 & 55.74 & 43.60 \\
%  \midrule
%   ReConsider$_{base,test_M=5}$ & 30.86 & 59.25 & 44.08 & 51.66 \\
%   ReConsider$_{base,test_M=3}$ & 31.55 & 35.83 & 64.03 & 49.93 \\
% ReConsider$_{base,test_M=2}$ & 32.66 & 25.44 & 74.88 & 50.16 \\
%  ReConsider$_{large,test_M=5}$ & 32.41  & 67.06 & 47.06 & 52.06 \\
%  ReConsider$_{large,test_M=3}$ & 33.83 & 33.70 & 67.24 & 50.47 \\
% ReConsider$_{large,test_M=2}$ & 33.74 & 23.88 & 76.62 & 50.25 \\
% \midrule
% ReConsider$_{full,test_M=2}$ & 35.21 & 25.73  & 71.50 & 48.62 \\
% ReConsider$_{full,test_M=3}$ & 35.79 & 35.84 & 59.73 & 47.79 \\
% ReConsider$_{full,test_M=5}$ & 35.62 & 60.19 & 39.20 & 49.69 \\
% % ReConsider$_{full,test_M=10}$ & 35.62 & 78.72 & 20.05 & 49.38 \\
% \midrule
% ReConsider$_{M=2}$ w/ sigmoid & 35.21 & 10.56  & 69.38 & 39.97 \\
% ReConsider$_{M=3}$ w/ sigmoid & 35.79 & 9.78 & 71.43 & 40.60 \\
% ReConsider$_{M=5}$ w/ sigmoid & 35.62 & 9.36  & 72.59 & 40.97 \\
% % \midrule
% % ReConsider$_{M=2}$ + TS &  &  &  & \\
% % ReConsider$_{M=3}$ + TS &  &  &  & \\
% % ReConsider$_{M=5}$ + TS &  &  &  & \\
% \midrule
%  ReConsider$_{M=5}$ + Aug  & 35.49 & 3.86 & 85.02 &  44.44 \\
%  ReConsider$_{M=5}$ + AnsEquiv + Aug & 35.73 & 2.77 & 85.84 & 44.31 \\
%  \bottomrule
% \end{tabular}}
%  \caption{Calibration results of representation-based calibrators.}
%  \label{tab:representation}
% \end{center}
% \end{table*}

%  \chenglei{The EM is way lower than expected. Maybe include some key features in the input as well? Do people know why neural rerankers don't work in this case?
%  For contrastive training, I'll just follow supervised SimCSE.
%  Possible reason: some questions have too many positives and dominate. Try: one positive with multiple negatives. Hyper-parameters. Directly try RECONSIDER? TODO: try classification datasets as well. Evaluation results under new metrics for different QA calibration methods.}


% \chen{We can combine table 4, 5 and 6 into one table, and for table 6, only include Joint approach.}

% \begin{table}[t]
% \small
% \begin{center}
% \setlength{\tabcolsep}{1.4mm}{
% \begin{tabular}{ c c c c c }
% \toprule
%   & EM & ICE$_{\mathrm{pos}}$ & ICE$_{\mathrm{neg}}$  & MacroCE \\ 
%   \midrule
%   No Calibration & 32.85 & 31.46 & 55.74 & 43.60 \\
%   \midrule
%  Softmax Confidence & 35.62 & 60.19 & 39.20 & 49.69 \\
%  Sigmoid Confidence & 35.62 & 9.37 & 72.59 & 40.97 \\
%  %Sigmoid + Augment & 35.49 & 3.86 & 85.02 & 44.44 \\
%  \bottomrule
% \end{tabular}}
%  \caption{Calibration results of using the neural answer reranker (ReConsider). We explore using either softmax or sigmoid to convert the raw reranker logits to confidence values.
% %  , and we also explore a data augmentation strategy for training the reranker. Only the sigmoid scoring without augmentation has some marginal improvement on MacroCE.
% The sigmoid scoring achieves marginal MacroCE improvement. 
%  }
%  \label{tab:reconsider}
% \end{center}
% \end{table}

% \chen{I removed the data augmentation part, more like a failed attempt to me. }

\subsection{Neural Reranker}

Instead of using manual features, an alternative approach is to train a neural answer reranker for post-hoc calibration. We adopt ReConsider~\cite{Iyer2020RECONSIDERRU} as our neural answer reranker, where we train a BERT-large classifier by feeding in the concatenation of the question, passage, and answer span. During training, for each question we include one randomly chosen positive and $M - 1 (M=10)$ randomly chosen hard negatives. We use DPR-BERT's predictions on NQ training set for reranker training. During inference, we use the trained reranker to rerank the top five predictions. 
%
We explore two ways of obtaining the confidence value of the top reranked answer prediction: 1) we computer softmax over the top $M=5$ predictions; 2) we compute sigmoid of the raw logit score. 
%Furthermore, we explore an additional data augmentation strategy for training the answer reranker. In particular, 
%we double the number of negative passages per question by 
%keeping the original question and passage but changing the answer to another span in the passage.

% \begin{itemize}
%     \item Keep the question, but change the passage-answer pair to another one with the same answer type and the replacement passage is retrieved so that it has high lexical overlap with the original passage (sampled from the training data).
    
%      \item Keep the question and passage, but change the answer to another span in the passage. 
    
%     % \item Keep the passage-answer pair, but change the question to another one with no answer overlap (the replacement question is retrieved from the training corpus). 
    
%     % \item Keep the passage-answer pair, remove keywords from the original question so that it lacks information and becomes unanswerable. 
    
% \end{itemize}

According to Table~\ref{tab:classifiers}, we find that the sigmoid scoring works better for calibration than softmax, but neural reranking is generally ineffective for improving MacroCE.
%we find that sigmoid scoring works better for calibration and data augmentation does not improve the calibration. Overall we conclude that this neural reranker approach is ineffective for improving MacroCE. 

% One could argue that the reason for the failure of the feature-based classifier is that the features alone do not tell information for distinguishing correct and wrong predictions. To remedy this, we also explore the possibility of learning more discriminative representations that can tell the differences between correct and wrong predictions. 
% We adopt ReConsider as the neural reranker. \chenglei{TODO: You guys can add some description about ReConsider. I will add in the more specific hyper-parameters later.}

% We start with a binary classification baseline where we finetune a RoBERTa-base classifier and then explore the a contrastive learning based approach with synthetic data augmentation. 


% \subsubsection{Binary Classification Baseline}

% We sample predictions on the NQ dev set as the training data for the classifier. Specifically, for each question, if there are positive predictions, we sample one positive prediction and 9 negative predictions to use as training data. We also hold-out 10\% such questions to use as dev data. This results in a training set of 4920 questions and dev set of 540 questions. 

% When sampling the negative predictions, we sample negative predictions with high confidence scores as hard negatives. We follow ReConsider's pipeline where we normalize across all candidate predictions of a question. 

% \chenglei{Sewon is right, the binary classification approach would not work. So we do it in ReConsider's style. It normalizes the positive and negative predictions of each question, then maximizes for the positive prob, which I think is inherently similar to a contrastive objective.}

% During testing, we consider two settings: 1) the joint calibration setup where we consider top-100 predictions for each test question; 2) the pipeline calibration setup where we consider the top-10 predictions from the top passage only. 

% \chenglei{TS on top of ReConsider. Try label smoothing? }


% Preliminary results:


% train\_M = 10, test\_M = 2: test EM = 32.66.

% train\_M = 10, test\_M = 3: test EM = 31.55.

% train\_M = 10, test\_M = 5: test EM = 30.86.

% train\_M = 24, test\_M = 2: test EM = 32.63.

% train\_M = 24, test\_M = 3: test EM = 31.80

% train\_M = 24, test\_M = 5: test EM = 30.80.

% BERT-large:

% train\_M = 10, test\_M = 2: test EM = 33.74.

% train\_M = 10, test\_M = 3: test EM = 33.10.

% train\_M = 10, test\_M = 5: test EM = 32.41. 


% Calibration results:

% base, train$_{M}$=10, test$_{M}$=5:

% EM: 30.859

% Acc:  [-1.0, -1.0, 0.36, 0.33, 0.33, 0.24, 0.26, 0.15, 0.25, 0.05]

% Conf:  [-1.0, -1.0, 0.27, 0.35, 0.45, 0.55, 0.65, 0.75, 0.85, 0.95]

% Sizes:  [0, 0, 539, 1307, 1011, 316, 183, 129, 85, 40]

% Interval-based ECE: 14.836

% base, train$_{M}$=10, test$_{M}$=3:

% EM: 31.551

% Acc:  [-1.0, -1.0, -1.0, 0.3, 0.32, 0.33, 0.28, 0.31, 0.31, 0.36]

% Conf:  [-1.0, -1.0, -1.0, 0.38, 0.46, 0.55, 0.65, 0.75, 0.84, 0.95]

% Sizes:  [0, 0, 0, 145, 727, 864, 600, 501, 409, 364]

% Interval-based ECE: 32.525


% base, train$_{M}$=10, test$_{M}$=2:

% EM: 32.659

% Acc:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.34, 0.32, 0.33, 0.32, 0.32]

% Conf:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.55, 0.65, 0.75, 0.85, 0.95]

% Sizes:  [0, 0, 0, 0, 0, 816, 715, 643, 623, 813]

% Interval-based ECE: 42.117


% large, train$_{M}$=10, test$_{M}$=5:

% EM: 32.410

% Acc:  [-1.0, -1.0, 0.34, 0.36, 0.38, 0.22, 0.22, 0.21, 0.2, 0.15]

% Conf:  [-1.0, -1.0, 0.27, 0.35, 0.45, 0.55, 0.65, 0.75, 0.85, 0.95]

% Sizes:  [0, 0, 438, 1189, 1068, 309, 214, 164, 133, 95]

% Interval-based ECE: 15.579

% large, train$_{M}$=10, test$_{M}$=3:

% EM: 33.102

% Acc:  [-1.0, -1.0, -1.0, 0.37, 0.35, 0.33, 0.35, 0.3, 0.34, 0.31]

% Conf:  [-1.0, -1.0, -1.0, 0.38, 0.46, 0.55, 0.65, 0.75, 0.85, 0.95]

% Sizes:  [0, 0, 0, 135, 605, 775, 611, 481, 456, 547]

% Interval-based ECE: 33.828

% large, train$_{M}$=10, test$_{M}$=2:

% EM: 33.740

% Acc:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.36, 0.34, 0.33, 0.36, 0.32]

% Conf:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.55, 0.65, 0.75, 0.85, 0.96]

% Sizes:  [0, 0, 0, 0, 0, 749, 687, 571, 599, 1004]

% Interval-based ECE: 42.710


% BERT-base trained on full NQ training data (train\_M = 10):

% test\_M = 2:

% EM: 35.208

% Acc:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.3, 0.36, 0.32, 0.35, 0.46]

% Conf:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.55, 0.65, 0.75, 0.85, 0.96]

% Sizes:  [0, 0, 0, 0, 0, 992, 770, 636, 578, 634]

% Interval-based ECE: 37.267

% Instance ECE: 55.386

% pos ECE:  25.732461013674868

% neg ECE:  71.49995637516832

% category-average ECE:  48.616208694421594


% test\_M = 3:

% EM: 35.789

% Acc:  [-1.0, -1.0, -1.0, 0.27, 0.29, 0.37, 0.34, 0.38, 0.43, 0.53]

% Conf:  [-1.0, -1.0, -1.0, 0.38, 0.45, 0.55, 0.65, 0.75, 0.85, 0.95]

% Sizes:  [0, 0, 0, 248, 880, 801, 635, 442, 326, 278]

% Interval-based ECE: 25.529

% Instance ECE: 51.183

% pos ECE:  35.8399870983242

% neg ECE:  59.73451125858206

% category-average ECE:  47.78724917845313


% test\_M = 5:

% EM: 35.623

% Acc:  [-1.0, -1.0, 0.28, 0.36, 0.45, 0.25, 0.3, 0.3, 0.32, 0.11]

% Conf:  [-1.0, -1.0, 0.27, 0.35, 0.45, 0.55, 0.64, 0.74, 0.85, 0.94]

% Sizes:  [0, 0, 781, 1386, 992, 224, 111, 63, 34, 19]

% Interval-based ECE: 5.414

% Instance ECE: 46.676

% pos ECE:  60.19041175648127

% neg ECE:  39.19835434910337

% category-average ECE:  49.69438305279232

% test\_M = 10:

% EM: 35.623

% Acc:  [-1.0, 0.32, 0.39, 0.49, 0.05, -1.0, -1.0, -1.0, -1.0, -1.0]

% Conf:  [-1.0, 0.16, 0.24, 0.32, 0.44, -1.0, -1.0, -1.0, -1.0, -1.0]

% Sizes:  [0, 1962, 1327, 302, 19, 0, 0, 0, 0, 0]

% Interval-based ECE: 15.540

% Instance ECE: 40.951

% pos ECE:  78.71524380485042

% neg ECE:  20.053356591924583

% category-average ECE:  49.3843001983875


% \textbf{Sigmoid + Temperature Scaling}:

% Bascially pushes everything into the extreme ends:

% (negative logits become smaller, positive logits become larger)

% testM = 5:

% best temp = 0.02

% EM: 35.623

% Acc:  [0.09, 0.12, 0.0, 0.5, 1.0, 0.0, 0.25, 0.0, 0.0, 0.41]

% Conf:  [0.0, 0.16, 0.23, 0.35, 0.5, 0.55, 0.66, 0.77, 0.85, 1.0]

% Sizes:  [567, 8, 3, 4, 1, 3, 4, 5, 5, 3010]

% Interval-based ECE: 51.148

% Instance ECE: 51.324

% pos ECE:  4.35786141596255

% neg ECE:  77.31321679192303

% category-average ECE:  40.835539103942786


% \chenglei{TODO: add dense retriever score. Filter out false negatives in reranking. Include numbers of incorporating alternative answers.  CCE numbers of using sigmoid in QA calibration. Label smoothing. }

% \paragraph{Synthetic Data Augmentation}

% Apart from vanilla ReConsider, we also explored a data augmentation strategy on top of conventional ReConsider training. 

% Apart from the feature based approach, we also explore a representation approach where we use contrastive training with data augmentation to obtain representations that can better discriminate between correct predictions and wrong predictions. 

\subsection{Label Smoothing}
Besides the post-hoc calibration approaches above,
%All the above techniques are considered post-hoc calibration because the underlying QA model is fixed and we change the confidence values post-hoc. 
another way of calibration is to train models that are inherently calibrated, and a representative approach is label smoothing~\cite{Pereyra2017RegularizingNN,Desai2020CalibrationOP}. 

In label smoothing, we assign the gold label with probability mass $\alpha$, and the rest classes $\frac{1 - \alpha}{|Y| - 1}$. We apply label smoothing on all three components of the ODQA pipeline: passage selection (where the first passage is gold, the rest $K - 1$ are false); span start and end position selection, both of which the gold class is the gold position, and false classes are the rest of the positions in the passage.  
We use $\alpha = 0.1$ in our experiments, and we find that the calibration results are largely insensitive to the choice of $\alpha$. 
%We have also tried other values of $\alpha$ and they do not make significant differences for calibration results.
We change the loss function from cross entropy to KL divergence with the label smoothed gold probability distribution. 

We compare the calibration results of the model trained without and with label smoothing, and we also explore applying temperature scaling on top of the model trained with label smoothing. According to  Table~\ref{tab:classifiers}, contrary to previous conclusion that label smoothing helps calibration measured by ECE~\cite{Desai2020CalibrationOP}, label smoothing is ineffective for calibration measured by MacroCE. 

% The results of models trained with label smoothing are shown in Table~\ref{tab:ls_joint} and Table~\ref{tab:ls_pipeline} for joint and pipeline calibration respectively. We further experiment temperature scaling on top of the label smoothing trained models, and the results are in Table~\ref{tab:ls_ts_joint} and Table~\ref{tab:ls_ts_pipeline} for joint and pipeline calibration respectively. 

% \begin{table}[t]
% \small
% \begin{center}
% \setlength{\tabcolsep}{2mm}{
% \begin{tabular}{ l c c c c }
%  \toprule
%  & EM & ICE$_{\mathrm{pos}}$ & ICE$_{\mathrm{neg}}$ & MacroCE \\ 
%  \midrule
%     \multicolumn{5}{l}{\textbf{\em No Label Smoothing}} \\
%     Joint  & 32.85  & 31.46 & 55.74 & 43.60 \\
%     Pipeline & 34.07  & 10.11 & 78.30 & 44.21 \\
%  \midrule
%     \multicolumn{5}{l}{\textbf{\em Label Smoothing}} \\
%     Joint  & 35.76  & 32.08 & 56.04 & 44.06 \\
%     Pipeline & 35.57  & 11.27 & 77.17 & 44.22 \\
%  \midrule
%     \multicolumn{5}{l}{\textbf{\em Label Smoothing + Temperature Scaling}} \\
%     Joint  & 35.76 & 55.72 & 29.52 & 42.62 \\
%     Pipeline & 35.57 & 58.07 & 30.45 & 44.26 \\
%  \bottomrule
% \end{tabular}}
%  \caption{
%  Calibration results of DPR-BERT trained without and with label smoothing, as well as applying temperature scaling on top of the model trained with label smoothing. 
%  Label smoothing gives slight improvement on model performance but not MacroCE.
%  }
%  \label{tab:label_smoothing}
% \end{center}
% \end{table}






\begin{comment}
\begin{table*}[t]
\small
\setlength\tabcolsep{5pt}
\centering
\begin{tabular}{ c c c c c c c c c c c c} 
 \toprule
 score & aggregation & probability & calibrator & temp & 
 EM & ECE\textsubscript{interval} & ECE\textsubscript{density} & ICE & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE
 \\
  \midrule
  score$_1$ & no & softmax & NO & -- & 35.10 & 16.55 & 16.55 & 44.84 & 40.30 & 47.29 & 43.79 \\
  score$_1$ & yes & softmax & NO & -- & 31.14 & 38.05  &  38.05 & 45.85  & 12.51  & 60.92 & 36.71 \\
   score$_1$ & no & sigmoid & NO & -- & 35.10 & 52.12 & 52.12 & 54.35 & 3.17 & 82.02 & 42.59  \\
  score$_1$ & yes & sigmoid & NO & -- & 31.14 & 52.74 & 52.74 & 54.61 & 3.01 & 77.94 & 40.47 \\
  \midrule
   score$_2$ & no & softmax & NO & -- & 35.76 & 24.53 & 24.53 & 47.47 & 32.08 & 56.04 & 44.06  \\
  score$_2$ & yes & softmax & NO & -- & 31.75 & 42.88 & 42.88 & 48.79 & 9.31 & 67.16 & 38.23 \\
   score$_2$ & no & sigmoid & NO & -- & 35.76 & 50.69 & 50.69 & 52.88 & 3.06 & 80.61 & 41.84 \\
  score$_2$ & yes & sigmoid & NO & -- & 31.72 & 51.64 & 51.64 & 53.21 & 2.47 & 76.78 & 39.62 \\
  \midrule
   score$_3$ & no & softmax & NO & -- & 35.76 & 34.69 & 34.69 & 36.03 & 98.88 & 1.04 & 49.96 \\
  score$_3$ & yes & softmax & NO & -- & 36.01 & 34.65 & 34.65 & 36.33 & 98.55 & 1.31 & 49.93 \\
   score$_3$ & no & sigmoid & NO & -- & 35.76 & 16.49 & 16.93 & 49.72 & 47.56 & 50.93 & 49.24  \\
  score$_3$ & yes & sigmoid & NO & -- & 36.01 & 16.36 & 17.45 & 49.67 & 47.37 & 50.97 & 49.17 \\
 \midrule
  score$_4$ & no & none & NO & -- &  35.76 & 29.92 & 29.84 & 34.62 & 90.13 & 3.73 & 46.93 \\
 \bottomrule
\end{tabular}
\caption{Joint calibration results on NQ test set without calibration. The model is trained with label smoothing ($\alpha = 0.9$).}
\label{tab:ls_joint}
\end{table*}




\begin{table*}[t]
\small
\setlength\tabcolsep{4pt}
\centering
\begin{tabular}{ c c c c c c c c c c c c} 
 \toprule
 score & aggregation & probability & calibrator & temp & 
 EM & ECE\textsubscript{interval} & ECE\textsubscript{density} & ICE & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE
 \\
  \midrule
  score$_1$ & no & softmax & NO & -- & 35.57 & 45.71 & 45.71 & 53.73 & 11.27 & 77.17 & 44.22 \\
  score$_1$ & yes & softmax & NO & -- & 34.43 & 46.72 & 46.72 & 54.35 & 11.08 & 77.08  & 44.08  \\
  score$_2$ & no & softmax & NO & -- & 35.57 & 45.71 & 45.71 & 53.73 & 11.27 & 77.17 & 44.22 \\
  score$_2$ & yes & softmax & NO & -- & 34.79 & 46.74 & 46.74 & 54.11 & 10.58 & 77.33 & 43.95 \\
  score$_5$ & no & softmax & NO & -- & 35.57 & 24.72 & 25.12 & 38.32 & 88.62 & 10.55 & 49.59 \\
  score$_5$ & yes & softmax & NO & -- & 35.57 & 24.21 & 24.39 & 38.44 & 88.07 & 11.04 & 49.56 \\
 score$_6$ & no & none & NO & -- & 35.57 & 27.11 & 27.06 & 34.45 & 86.47 & 5.73 & 46.10 \\
 \bottomrule
\end{tabular}
\caption{Pipeline calibration on NQ test set. The model is trained with label smoothing ($\alpha = 0.9$). }
\label{tab:ls_pipeline}
\end{table*}




\begin{table*}[t]
\small
\setlength\tabcolsep{5pt}
\centering
\begin{tabular}{ c c c c c c c c c c c c} 
 \toprule
 score & aggregation & probability & calibrator & temp & 
 EM & ECE\textsubscript{interval} & ECE\textsubscript{density} & ICE & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE
 \\
  \midrule
  score$_1$ & no & softmax & TS & 1.60 & 35.10 & 6.88 & 6.59 & 38.85 & 56.84 & 29.12 & 42.98 \\
  score$_1$ & yes & softmax & TS & 3.09 & 31.14 & 6.76 & 7.09 & 29.18 & 47.89 & 20.72 & 34.30 \\
   score$_1$ & no & sigmoid & TS & 10.00 & 35.10 & 25.39 & 25.35 & 50.09 & 35.64 & 57.91 & 46.77 \\
  score$_1$ & yes & sigmoid & TS & 10.00 & 31.14 & 32.82 & 32.82 & 49.24 & 26.37 & 59.78 & 42.97 \\
  \midrule
   score$_2$ & no & softmax & TS & 2.01 & 35.76 & 7.44 & 7.17 & 38.89 & 55.72 & 29.52 & 42.62 \\
  score$_2$ & yes & softmax & TS & 4.06 & 31.75 & 7.55 & 7.34 & 28.81 & 46.68 & 20.50 & \textbf{33.59} \\
   score$_2$ & no & sigmoid & TS & 10.00 & 35.76 & 28.23 & 28.23 & 49.66 & 29.96 & 60.63 & 45.29 \\
  score$_2$ & yes & sigmoid & TS & 10.00 & 31.75 & 36.60 & 36.60 & 49.07 & 19.63 & 62.76 & 41.20 \\
  \midrule
   score$_3$ & no & softmax & TS & 0.02 & 35.76 & 27.15 & 26.62 & 33.32 & 69.10 & 13.40 & 41.25 \\
  score$_3$ & yes & softmax & TS & 0.02 & 36.01 & 25.10 & 25.10 & 32.45 & 63.12 & 15.19 & 39.16 \\
   score$_3$ & no & sigmoid & TS & 10.00 & 35.76 & 14.39 & 17.34 & 49.97 & 49.75 & 50.09 & 49.92 \\
  score$_3$ & yes & sigmoid & TS & 10.00 & 36.01 & 14.15 & 18.17 & 49.97 & 49.73 & 50.10 & 49.92 \\
 \midrule
  score$_4$ & no & none & TS & 0.45 & 35.76 & 20.99 & 20.94 & 37.42 & 66.97 & 20.98 & 43.97 \\
 \bottomrule
\end{tabular}
\caption{Joint calibration results on NQ test set with additional temperature scaling. The model is trained with label smoothing ($\alpha = 0.9$). We apply additional temperature scaling on top of the label smoothed model. The temperature is tuned to optimize interval ECE on the NQ dev set.}
\label{tab:ls_ts_joint}
\end{table*}




\begin{table*}[t]
\small
\setlength\tabcolsep{4pt}
\centering
\begin{tabular}{ c c c c c c c c c c c c} 
 \toprule
 score & aggregation & probability & calibrator & temp & 
 EM & ECE\textsubscript{interval} & ECE\textsubscript{density} & ICE & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE
 \\
  \midrule
  score$_1$ & no & softmax & TS & 4.66 & 35.57 & 4.63 & 4.93 & 40.27 & 58.07 & 30.45 & 44.26 \\
  score$_1$ & yes & softmax & TS & 4.67 & 34.43 & 3.88 & 4.29 & 40.05 & 57.12 & 31.08 & 44.10 \\
  score$_2$ & no & softmax & TS & 4.66 & 35.57 & 4.63 & 4.93 & 40.27 & 58.07 & 30.45 & 44.26 \\
  score$_2$ & yes & softmax & TS & 4.78 & 34.79 & 5.04 & 4.68 & 40.03 & 57.22 & 30.86 & 44.04 \\
  score$_5$ & no & softmax & TS & 0.07 & 35.57 & 13.89 & 13.73 & 36.18 & 61.76 & 22.06 & 41.91 \\
  score$_5$ & yes & softmax & TS & 0.07 & 35.57 & 13.35 & 13.00 & 36.32 & 60.94 & 22.73 & 41.84 \\
 score$_6$ & no & none & TS & 0.60 & 35.57 & 18.86 & 18.54 & 36.18 & 70.24 & 17.38 & 43.81 \\
 \bottomrule
\end{tabular}
\caption{Pipeline calibration on NQ test set with additional temperature scaling. The model is trained with label smoothing ($\alpha = 0.9$). We apply additional temperature scaling on top of label smoothed models. The temperature is tuned to optimize interval ECE on the NQ dev set.}
\label{tab:ls_ts_pipeline}
\end{table*}

\end{comment}

% \chen{For table 7, only show ICE (POS, NEG) and MarcoCE}


% \begin{table*}[t]
% \small
% \setlength\tabcolsep{5pt}
% \centering
% \begin{tabular}{ c c c c c c c c } 
%  \toprule
%  Calibrator &  
%  EM & ECE\textsubscript{interval} & ECE\textsubscript{density} & ICE & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE
%  \\
%   \midrule
%   \multicolumn{8}{l}{\textbf{\em No Calibration}} \\
%   Joint & 36.45 & 31.63 & 31.62 & 36.88 & 93.96 & 4.14  & 49.05  \\
%     Pipeline & 37.17 & 51.72 & 51.72  & 55.69  & 5.33  & 85.48 &  45.41 \\
%     \midrule
% \multicolumn{8}{l}{\textbf{\em Binary Baseline}} \\
%     Joint & 36.45 & 40.06 & 37.67 & 40.06 & 55.78 & 31.04 & 43.41 \\
%     Pipeline & 37.17 & 32.85 & 31.14 & 32.85 & 45.08 & 25.62 & 35.35 \\
% \midrule
% \multicolumn{8}{l}{\textbf{\em Average Baseline}} \\
%     Joint & 36.45 & 1.45 & 2.11 & 45.94 & 65.00 & 35.00 & 50.00 \\
%     Pipeline & 37.17 & 0.68 & 2.16 & 46.53 & 63.51 & 36.49 & 50.00 \\
% \midrule
% \multicolumn{8}{l}{\textbf{\em Random Confidence Baseline}} \\
%      Joint & 36.45 & 27.68 & 27.50 & 50.31 & 50.70 & 50.09 & 50.40 \\
%     Pipeline & 37.17 & 27.96 & 27.77 & 50.68 & 51.19 & 50.39 & 50.79 \\
% \midrule
% \multicolumn{8}{l}{\textbf{\em Temperature Scaling}} \\
% Joint & 36.45 & 6.33 & 6.39 & 39.59 & 56.12 & 30.11 & 43.12 \\
%  Pipeline & 37.17 & 4.37 & 4.73 & 41.10 & 58.35 & 30.89 & 44.62 \\
% \midrule
% \multicolumn{8}{l}{\textbf{\em Consistency Calibration (Binary)}} \\
% Joint & 36.45 & 32.35 & 30.03 & 32.35 & 32.52 & 32.26  & 32.39 \\
% Pipeline & 37.17 & 31.83 & 30.11 & 31.83 & 30.77 & 32.45 & 31.61 \\
% \midrule
% \multicolumn{8}{l}{\textbf{\em Consistency Calibration (Frequency)}} \\
% Joint & 36.45 & 23.15 & 22.58 & 38.61 & 27.36 & 45.07 & 36.21 \\
% Pipeline & 37.17 & 21.85 & 21.98 & 37.81 & 26.48 & 44.51 & 35.50 \\
% \midrule
% \multicolumn{8}{l}{\textbf{\em Consistency Calibration (Classifier)}} \\
% Joint  & 36.56 & 31.52 & 29.64 & 31.52 & 31.38 & 31.60 & 31.49 \\
% Pipeline & 37.17 & 31.33 & 29.17 & 31.33 & 31.45 & 31.26 & 31.35 \\
%  \bottomrule
% \end{tabular}
% \caption{Calibration results of baseline calibration methods as well as our new consistency calibration. We highlight the best result in bold. Our new consistency calibration method  outperforms all other baselines on MacroCE. Note that different metrics give different ranking of these methods, which further highlights the importance of using a reliable and informative metric. }
% \label{tab:consistency}
% \end{table*}




\begin{table*}[t]
\small
\setlength\tabcolsep{5pt}
\centering
\begin{tabular}{ c c c c c c | c c c c c} 
& \multicolumn{5}{c}{IID (NQ)} & \multicolumn{5}{c}{OOD (HotpotQA)} \\
 \toprule
 Calibrator &  
 EM & ECE\textsubscript{interval} & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE & EM & ECE\textsubscript{interval} & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE
 \\
  \midrule
  \multicolumn{8}{l}{\textbf{\em No Calibration}} \\
   Joint & 35.24 & 30.41 & 27.17 & 61.74 & 44.46 & 24.50 & 44.40 & 25.38 & 67.04 & 46.21 \\
    Pipeline & 36.34 & 50.08 & 6.93 & 82.63 & 44.78  & 22.78 & 61.22 & 12.48 & 82.95 & 47.72 \\
    \midrule
\multicolumn{8}{l}{\textbf{\em Binary Baseline}} \\
    Joint & 35.24 & 38.03 & 53.22 & 29.77 & 41.50 & 24.50 & 38.62 & 55.81 & 33.05 & 44.43 \\
    Pipeline & 36.34 & 33.68 & 46.34 & 26.46 & 36.40  & 22.78 & 38.82 & 55.45 & 33.92 & 44.68 \\
\midrule
\multicolumn{8}{l}{\textbf{\em Average Baseline}} \\
    Joint & 35.24 & 2.00 & 64.25 & 35.75 & 50.00 & 24.50 & 11.25 & 64.25 & 35.75 & 50.00 \\
    Pipeline & 36.34 & 0.03 & 63.66 & 36.34 & 50.00 & 22.78 & 13.56 & 63.66 & 36.34 & 50.00 \\
\midrule
\multicolumn{8}{l}{\textbf{\em Temperature Scaling}} \\
Joint &  &   &  &  &  \\
 Pipeline &  &  &  &  &  \\
 \midrule
\multicolumn{8}{l}{\textbf{\em Feature-based Classifier (LR)}} \\
Joint  \\
 Pipeline  \\
  \midrule
\multicolumn{8}{l}{\textbf{\em Feature-based Classifier (SVM)}} \\
Joint  \\
 Pipeline  \\
  \midrule
\multicolumn{8}{l}{\textbf{\em Feature-based Classifier (RF)}} \\
Joint  \\
 Pipeline  \\
 \midrule
\multicolumn{8}{l}{\textbf{\em Neural Reranker (ReConsider)}} \\
Joint  \\
 Pipeline  \\
 \midrule
\multicolumn{8}{l}{\textbf{\em Label Smoothing}} \\
Joint  \\
 Pipeline  \\
  \midrule
\multicolumn{8}{l}{\textbf{\em Ensemble Calibration}} \\
Joint  \\
 Pipeline  \\
\midrule
\multicolumn{8}{l}{\textbf{\em Consistency Calibration (Binary)}} \\
Joint &  35.24 & 31.91 & 26.10 & 35.07 & 30.59 & 24.50 & 40.37 & 34.29 & 42.35 & 38.32 \\
Pipeline & 36.34 & 31.30 & 25.91 & 34.38 & 30.15 & 22.78 & 43.25 & 37.00 & 45.09 & 41.05 \\
\midrule
\multicolumn{8}{l}{\textbf{\em Consistency Calibration (Frequency)}} \\
Joint & 35.24 & 44.46 & 26.39 & 44.68 & 35.53 & 24.50 & 46.21 & 31.72 & 49.89 & 40.81 \\
Pipeline & 36.34 & 44.78 & 26.04 & 43.78 & 34.91 & 22.78 & 47.72 & 32.34 & 51.87 & 42.11 \\
\midrule
\multicolumn{8}{l}{\textbf{\em Consistency Calibration (Classifier)}} \\
Joint & 35.24 & 31.63 & 27.28 & 34.00 & 30.64 & 24.50 & 40.34 & 35.56 & 41.90 & 38.73 \\
Pipeline & 36.34 & 33.16 & 25.84 & 37.34 & 31.59 & 22.78 & 44.60 & 31.81 & 48.38 & 40.09 \\
 \bottomrule
\end{tabular}
\caption{Calibration results of baseline calibration methods as well as our new consistency calibration. We highlight the best result in bold. Our new consistency calibration method  outperforms all other baselines on MacroCE. Note that different metrics give different ranking of these methods, which further highlights the importance of using a reliable and informative metric. }
\label{tab:consistency}
\end{table*}



==> sections/archived/60-new-method.tex <==
% \chen{I think this section misses the intuition part. We need a few paragraphs saying why methods in section 5 do not work well, and the proposed approach works. }

% We first reflect the failure of existing calibration methods in section~\ref{sec:re-eval}. 
The failure of temperature scaling under MacroCE suggests that directly relying on the outputs from QA model is not sufficient for calibration. This calls for additional cues that can expose the model's confidence. We take inspiration from training dynamics~\cite{Swayamdipta2020DatasetCM}, which tracks whether the model makes consistent and correct predictions across the training process. While \citet{Swayamdipta2020DatasetCM} aim to measure the difficulty of the examples, we leverage similar intuition but focus on the calibration perspective.\footnote{Note that in \citet{Swayamdipta2020DatasetCM}, confidence is defined as the mean probability of the true label across epochs; our confidence scoring will be different from their definition.  Moreover, our definition of consistency is similar to they called `variability'.}

% \chen{I suggest the following from the motivation of Cartography paper: 1) both Post-hoc and label smoothing approaches are affected by training data quality 2) existing datasets contain noise, so models are easy to make high confidence on wrong predictions 3) However, we think (from the conclusion of Cartography paper ) under such scenarios, the predictions would be unstable over checkpoints, that's why we make decisions based on prediction consistency.}

% In previous sections, we have shown that existing calibration methods fail to bring significant improvement on MacroCE. 
Specifically, 
 we propose a new simple calibration method called \textbf{consistency calibration}. 
 The idea is that if the same answer prediction is consistent throughout the training trajectory, then it could serve as a strong sign that the model is confident about that prediction, and vice versa. 
 
To implement this idea, we save a total of eight checkpoints throughout training.
%($c$ is a hyper-parameter that can be tuned), each checkpoint being equally (in this experiment 12k steps) apart. 
 %
We take the final checkpoint as the QA model for evaluation. For each question, we check how many times the predicted answer string also appears from the previous seven checkpoints ($n \in [0,7]$).
%we denote this integer $n \in [0,7]$. 
For calibration, we set a threshold $n_0$ and for all predictions with $n \ge n_0$, we assign a confidence value of 1, otherwise 0. We iterate through all possible threshold values on the NQ development set and select the best $n_0$ that minimizes the MacroCE. We call this implementation Binary Consistency Calibration. 
%We then directly apply this tuned threshold value on the NQ test set for calibration evaluation. 

We also explore two other alternative implementations of consistency calibration. The first one is Frequency-based Consistency Calibration where the confidence of each prediction is computed as $\frac{n}{7}$ where $n$ is the number of times that the prediction was made by the 7 intermediate checkpoints. The second one is Classifier-based Consistency Calibration where we treat whether the final prediction is also predicted by each intermediate checkpoint as a binary feature, and train a linear classifier on such 7-dimensional feature vectors to predict the correctness of the final prediction. 

% Linear classifier weights for the 7 checkpoints:
% coefs:  [[0.42213862 0.22641724 0.31732398 0.40452891 0.39299144 0.28919917
%   0.63056155]]
 
 We compare two ways of obtaining the top prediction of each checkpoint - joint (considering top predictions from all top-10 retrieved passages) and pipeline (only considering the top predictions from top-1 retrieved passage). 
%  We use Joint S+E+P as the scoring function with no answer aggregation when deciding the top prediction.
 %Apart from the baseline without calibration and the temperature scaling baseline, 
 We also compare with the following other simple baselines to ensure that our claimed improvement on MacroCE is indeed meaningful:
 
 \sewon{Proposal: A bit weird to have these trivial references later. Shouldn't it be introduced when the metric was introduced, or at least when we discuss results in the end of Section 4 or Section 5?}
 \chenglei{How about we combine Table 4 \& 5 so all these are baselines.}
 \sewon{Another thought 1: I would delete random confidence baseline if we need to save space because it is clearly worse than other two.}
 \chenglei{Make sense.}
 \sewon{Another thought 2: Binary and Average baselines are not bad because the dev and the test distributions are similar. What about we add one OOD dataset? I think these methods will have worse OOD result.}
 \chenglei{We can, although if we are going to add OOD, we might need to add OOD evaluation results for all methods in Table 5. Maybe we can discuss this later in the meeting?}
 \sewon{Another thought 3: Rename `Average baseline' into `Constant baseline' to make naming consistent to `Binary baseline'? Or maybe both names are not super intuitive.. I'll think more.}
 \chenglei{Feel free to do naming changes.}
 
\begin{itemize}
    \item Binary baseline: We assign the top p\% (p\% is the model accuracy on the development set) confident predictions in the test set with confidence value of 1, and others 0.  
    
    \item Average baseline: We assign all predictions in the test set with the confidence value equal to the average accuracy on the development set.
    
    % \item random binary baseline: We randomly assign each test prediction with a confidence value of 0 or 1. 
    
    \item Random confidence baseline: For each test prediction, we assign the prediction with a random confidence value drawn uniformly from the range $[0,1]$. 
\end{itemize}

According to Table~\ref{tab:consistency}, our consistency calibration achieves the best MacroCE compared to all other baseline calibration methods. We believe that it is possible to develop more sophisticated calibration methods based on our consistency idea to further improve the calibration performance, and we leave it to future work. 

% \section{Trivial Baselines}

% \chenglei{Feel free to change the naming! And we need to find a place to put this section.}

% We experiment several trivial baselines to better understand our various metrics. Specifically, we explore the following baselines:



% The results are in Table~\ref{tab:results_trivial}.

 
%  The results are shown in Table~\ref{tab:results_consistency}. 
 
 
%  \chenglei{ Apart from this thresholding baseline, other methods are possible such as training a linear classifier based on the checkpoint consistency statistics (so that we might assign higher weight to later checkpoint, for instance). We can also assign continuous confidence values based on the number of occurrences. I will try some of those this week and add in the results here, before that you can go ahead and write about the current results.}
 





% \begin{table*}[t]
% \small
% \setlength\tabcolsep{4pt}
% \centering
% \begin{tabular}{ c c c c c c c c } 
%  \toprule
%  calibrator &  
%  EM & ECE\textsubscript{interval} & ECE\textsubscript{density} & ICE & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE
%  \\
%   \midrule
%   No$_{\mathrm{joint}}$ & 36.45 & 31.63 & 31.62 & 36.88 & 93.96 & 4.14  & 49.05  \\
%   No$_{\mathrm{pipeline}}$ & 37.17 & 51.72 & 51.72  & 55.69  & 5.33  & 85.48 &  45.41 \\
%   TS$_{\mathrm{joint}}$ & 36.45 & 6.33 & 6.39 & 39.59 & 56.12 & 30.11 & 43.12 \\
%   TS$_{\mathrm{pipeline}}$ & 37.17 & 4.37 & 4.73 & 41.10 & 58.35 & 30.89 & 44.62 \\
%   Consistency$_{\mathrm{joint}}$ & 36.45 & 32.35 & 30.03 & 32.35 & 32.52 & 32.26  & 32.39 \\
%   Consistency$_{\mathrm{pipeline}}$ & 37.17 & 31.83 & 30.11 & 31.83 & 30.77 & 32.45 & 31.61 \\
%  \bottomrule
% \end{tabular}
% \caption{Results for our consistency calibration. All results are reported on the test set. The best threshold $n_0$ is 5 for both joint calibration and pipeline calibration. The optimal temperature for joint calibration is 2.65 and for pipeline calibration the tuned temperature is 7.39.}
% \label{tab:results_consistency}
% \end{table*}





==> sections/other-tasks.tex <==
\section{Beyond ODQA}

We try calibration on two other tasks: sentiment analysis (SST-2) and NLI (SNLI-30K). We use RoBERTa-base for finetuning. 

SST-2 before calibration:

\#test questions:  1821

EM: 94.838

Acc:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.25, 0.6, 0.5, 0.59, 0.96]

Conf:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.56, 0.65, 0.75, 0.87, 1.0]

Sizes:  [0, 0, 0, 0, 0, 4, 5, 8, 22, 1782]

Interval-based ECE: 4.426

Instance ECE: 5.339

pos ECE:  0.4816123289252957

neg ECE:  94.58563486312298

category-average ECE:  47.533623596024135

SST-2 after TS (Optimize category-ECE on the dev set):

best temperature = 3.25

EM:  94.838

Acc:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.44, 0.65, 0.73, 0.96, 1.0]

Conf:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.55, 0.65, 0.76, 0.88, 0.9]

Sizes:  [0, 0, 0, 0, 0, 16, 31, 71, 1547, 156]

Interval-based ECE:  7.943

pos ECE: 12.16

neg ECE: 78.27

category-average: 45.21


SST-2 after TS (Optimize interval-ECE on the dev set):

best temperature = 2.24

EM:  94.838

Acc:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.44, 0.56, 0.66, 0.76, 0.97]

Conf:  [-1.0, -1.0, -1.0, -1.0, -1.0, 0.55, 0.65, 0.75, 0.86, 0.95]

Sizes:  [0, 0, 0, 0, 0, 9, 16, 32, 83, 1681]

dev ECE:  2.466

pos ECE: 5.64

neg ECE: 85.08

category-average: 45.36







\begin{table*}[t]
\small
\setlength\tabcolsep{4pt}
\centering
\begin{tabular}{ c c c c c c c c } 
 \toprule
 calibrator &  
 EM & ECE\textsubscript{interval} & ECE\textsubscript{density} & ICE & ICE\textsubscript{pos} & ICE\textsubscript{neg} & MacroCE
 \\
  \midrule
   No$_{\mathrm{joint}}$ & 36.45 & 31.63 & 31.62 & 36.88 & 93.96 & 4.14  & 49.05  \\
    No$_{\mathrm{pipeline}}$ & 37.17 & 51.72 & 51.72  & 55.69  & 5.33  & 85.48 &  45.41 \\
    Binary$_{\mathrm{joint}}$ & 36.45 & 40.06 & 37.67 & 40.06 & 55.78 & 31.04 & 43.41 \\
    Binary$_{\mathrm{pipeline}}$ & 37.17 & 32.85 & 31.14 & 32.85 & 45.08 & 25.62 & 35.35 \\
    Average$_{\mathrm{joint}}$ & 36.45 & 1.45 & 2.11 & 45.94 & 65.00 & 35.00 & 50.00 \\
    Average$_{\mathrm{pipeline}}$ & 37.17 & 0.68 & 2.16 & 46.53 & 63.51 & 36.49 & 50.00 \\
     Random$_{\mathrm{joint}}$ & 36.45 & 27.68 & 27.50 & 50.31 & 50.70 & 50.09 & 50.40 \\
    Random$_{\mathrm{pipeline}}$ & 37.17 & 27.96 & 27.77 & 50.68 & 51.19 & 50.39 & 50.79 \\
 \bottomrule
\end{tabular}
\caption{Results for our trivial baselines. All results are on the NQ test set. Joint EM on the NQ dev set is 35.83. Pipeline EM on the NQ dev set is 36.49. }
\label{tab:results_trivial}
\end{table*}


\section{Trivial Baselines}

\chenglei{Feel free to change the naming! And we need to find a place to put this section.}

We experiment several trivial baselines to better understand our various metrics. Specifically, we explore the following baselines:

\begin{itemize}
    \item binary baseline: Suppose the model accuracy is p\% on the dev set, we assign the top p\% most confident predictions in the test set with confidence value of 1, and others 0.  
    
    \item average baseline: We assign all predictions in the test set with the confidence value equal to the average accuracy on the dev set.
    
    % \item random binary baseline: We randomly assign each test prediction with a confidence value of 0 or 1. 
    
    \item random confidence baseline: For each test prediction, we assign the prediction with a random confidence value drawn uniformly from the range $[0,1]$. 
\end{itemize}



The results are in Table~\ref{tab:results_trivial}.
